Safe Load Balancing in Software-Defined-Networking

High performance, reliability and safety are crucial properties of any Software-Defined-Networking (SDN) system. Although the use of Deep Reinforcement Learning (DRL) algorithms has been widely studied to improve performance, their practical applications are still limited as they fail to ensure safe operations in exploration and decision-making. To fill this gap, we explore the design of a Control Barrier Function (CBF) on top of Deep Reinforcement Learning (DRL) algorithms for load-balancing. We show that our DRL-CBF approach is capable of meeting safety requirements during training and testing while achieving near-optimal performance in testing. We provide results using two simulators: a flow-based simulator, which is used for proof-of-concept and benchmarking, and a packet-based simulator that implements real protocols and scheduling. Thanks to the flow-based simulator, we compared the performance against the optimal policy, solving a Non Linear Programming (NLP) problem with the SCIP solver. Furthermore, we showed that pre-trained models in the flow-based simulator, which is faster, can be transferred to the packet simulator, which is slower but more accurate, with some fine-tuning. Overall, the results suggest that near-optimal Quality-of-Service (QoS) performance in terms of end-to-end delay can be achieved while safety requirements related to link capacity constraints are guaranteed. In the packet-based simulator, we also show that our DRL-CBF algorithms outperform non-RL baseline algorithms. When the models are fine-tuned over a few episodes, we achieved smoother QoS and safety in training, and similar performance in testing compared to the case where models have been trained from scratch.

==> biblio.tex <==
@book{suttonReinforcementLearningIntroduction2018,
  title = {Reinforcement Learning: An Introduction},
  shorttitle = {Reinforcement Learning},
  author = {Sutton, Richard S. and Barto, Andrew G.},
  year = {2018},
  series = {Adaptive Computation and Machine Learning Series},
  edition = {2nd},
  publisher = {{The MIT Press}},
  address = {{Cambridge, Massachusetts}},
  abstract = {"Reinforcement learning, one of the most active research areas in artificial intelligence, is a computational approach to learning whereby an agent tries to maximize the total amount of reward it receives while interacting with a complex, uncertain environment. In Reinforcement Learning, Richard Sutton and Andrew Barto provide a clear and simple account of the field's key ideas and algorithms."--},
  isbn = {978-0-262-03924-6},
  langid = {english},
  lccn = {Q325.6 .R45 2018},
  keywords = {Reinforcement learning},
  file = {C\:\\Users\\lwx1222086\\Zotero\\storage\\QZREQM8P\\Sutton and Barto - 2018 - Reinforcement learning an introduction.pdf}
}

@inproceedings{gao2006avoiding,
  title={Avoiding oscillations due to intelligent route control systems.},
  author={Gao, Ruomei and Dovrolis, Constantinos and Zegura, Ellen W},
  booktitle={INFOCOM},
  year={2006}
}

@article{huangProactiveLoadBalancing2022,
  title = {Proactive {{Load Balancing Through Constrained Policy Optimization}} for {{Ultra-Dense Networks}}},
  author = {Huang, Miaona and Chen, Jun},
  year = {2022},
  month = oct,
  journal = {IEEE Communications Letters},
  volume = {26},
  number = {10},
  pages = {2415--2419},
  issn = {1558-2558},
  doi = {10.1109/LCOMM.2022.3190284},
  abstract = {Designing an intelligent self-organizing network (SON) architecture is challenging for future wireless networks. To meet the needs of SON, the reactive self-organizing model of the traditional network needs to be transformed into an active and interactive one. Due to the user mobility and small coverage of cells in ultra-dense networks (UDNs), the network load usually becomes unbalanced, leading to deteriorated network performance, such as low throughput, radio link failure, and poor user experience. Therefore, the technique of mobility load balancing (MLB) is critical to ensuring a seamless user experience among cells. This letter proposes an active and interactive MLB strategy for UDNs, which transforms the original reactive MLB into a forward-aware and active one. In particular, user mobility is first predicted based on the Bayesian additive regression tree (BART). Then, with the mobility predictions, the joint mobility robust optimization and MLB problem subject to users' rate constraint is solved via safe reinforcement learning. The pertaining simulation results show that the proposed method can improve the network performance and realize intelligent mobile management for future UDNs.},
  keywords = {Bayesian additive regression tree,constrained policy optimization,Handover,Load management,Load modeling,mobility load balancing,Optimization,Quality of service,Regression tree analysis,Reinforcement learning,ultra-dense networks}
}



@article{achiamConstrainedPolicyOptimization2017a,
  author       = {Joshua Achiam and
                  David Held and
                  Aviv Tamar and
                  Pieter Abbeel},
  title        = {{Constrained Policy Optimization}},
  journal      = { Computing Research Repository (CoRR)},
  volume       = {abs/1705.10528},
  year         = {2017},
  eprinttype    = {arXiv},
  eprint       = {1705.10528},
  timestamp    = {Mon, 13 Aug 2018 16:47:33 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/AchiamHTA17.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{achiamConstrainedPolicyOptimization2017ab,
  title = {Constrained {{Policy Optimization}}},
  booktitle = {Proceedings of the 34th {{International Conference}} on {{Machine Learning}}},
  author = {Achiam, Joshua and Held, David and Tamar, Aviv and Abbeel, Pieter},
  year = {2017},
  month = jul,
  pages = {22--31},
  publisher = {{PMLR}},
  issn = {2640-3498},
  urldate = {2023-05-30},
  abstract = {For many applications of reinforcement learning it can be more convenient to specify both a reward function and constraints, rather than trying to design behavior through the reward function. For example, systems that physically interact with or around humans should satisfy safety constraints. Recent advances in policy search algorithms (Mnih et al., 2016, Schulman et al., 2015, Lillicrap et al., 2016, Levine et al., 2016) have enabled new capabilities in high-dimensional control, but do not consider the constrained setting. We propose Constrained Policy Optimization (CPO), the first general-purpose policy search algorithm for constrained reinforcement learning with guarantees for near-constraint satisfaction at each iteration. Our method allows us to train neural network policies for high-dimensional control while making guarantees about policy behavior all throughout training. Our guarantees are based on a new theoretical result, which is of independent interest: we prove a bound relating the expected returns of two policies to an average divergence between them. We demonstrate the effectiveness of our approach on simulated robot locomotion tasks where the agent must satisfy constraints motivated by safety.},
  langid = {english},
  file = {C\:\\Users\\lwx1222086\\Zotero\\storage\\9LIGF8FK\\Achiam et al_2017_Constrained Policy Optimization.pdf}
}

@InProceedings{RILNET,
author="Lin, Qinliang
and Gong, Zhibo
and Wang, Qiaoling
and Li, Jinlong",
editor="Renault, {\'E}ric
and M{\"u}hlethaler, Paul
and Boumerdassi, Selma",
title={{RILNET: A Reinforcement Learning Based Load Balancing Approach for Datacenter Networks}},
booktitle="Machine Learning for Networking",
year="2019",
doi = {10.1007/978-3-030-19945-6_4},
publisher="Springer International Publishing",
address="Cham",
pages="44--55",
abstract="Modern datacenter networks are facing various challenges, e.g., highly dynamic workloads, congestion, topology asymmetry. ECMP, as a traditional load balancing mechanism which is widely used in today's datacenters, can balance load poorly and lead to congestion. Variety of load balancing schemes are proposed to address the problems of ECMP. However, these traditional schemes usually make load balancing decision only based on network knowledge for a snapshot or a short time past. In this paper, we propose a Reinforcement Learning (RL) based approach, called RILNET (ReInforcement Learning NETworking), aiming at load balancing for datacenter networks. RILNET employs RL to learn a network and control it based on the learned experience. To achieve a higher granularity of control, RILNET is constructed to route flowlet rather than flows. Moreover, RILNET makes routing decisions for aggregation flows (an aggregation flow is a flow set that includes all flows flowing from the same source edge switch to the same destination edge switch) instead of a single flow. In order to test performance of RILNET, we propose a flow-level simulation and a packet-level simulation, and the both results show that RILNET can balance traffic load much more effectively than ECMP and another load balancing solution, i.e., DRILL. Compared with DRILL, RILNET outperforms DRILL in data loss and maximal link delay. Specifically, the maximal link data loss and the maximal link delay of RILNET are 44.4{\%} and 25.4{\%} smaller than DRILL, respectively.",
isbn="978-3-030-19945-6"
}


@journal{linRILNETReinforcementLearning2019,
  title = {{{RILNET}}: {{A Reinforcement Learning Based Load Balancing Approach}} for {{Datacenter Networks}}},
  shorttitle = {{{RILNET}}},
  booktitle = {{Machine Learning for Networking}},
  author = {Lin, Qinliang and Gong, Zhibo and Wang, Qiaoling and Li, Jinlong},
  editor = {Renault, {\'E}ric and M{\"u}hlethaler, Paul and Boumerdassi, Selma},
  year = {2019},
  series = {Lecture {{Notes}} in {{Computer Science}}},
  pages = {44--55},
  publisher = {{Springer International Publishing}},
  address = {{Cham}},
  doi = {10.1007/978-3-030-19945-6_4},
  abstract = {Modern datacenter networks are facing various challenges, e.g., highly dynamic workloads, congestion, topology asymmetry. ECMP, as a traditional load balancing mechanism which is widely used in~today's datacenters, can balance load poorly and lead to congestion. Variety of load balancing schemes are proposed to address the problems of ECMP. However, these traditional schemes usually make load balancing decision only based on network knowledge for a snapshot or a short time past. In this paper, we propose a Reinforcement Learning (RL) based approach, called RILNET (ReInforcement Learning NETworking), aiming at load balancing for datacenter networks. RILNET employs RL to learn a network and control it based on the learned experience. To achieve a higher granularity of control, RILNET is constructed to route flowlet rather than flows. Moreover, RILNET makes routing decisions for aggregation flows (an aggregation flow is a flow set that includes all flows flowing from the same source edge switch to the same destination edge switch) instead of a single flow. In order to test performance of RILNET, we propose a flow-level simulation and a packet-level simulation, and the both results show that RILNET can balance traffic load much more effectively than ECMP and another load balancing solution, i.e., DRILL. Compared with DRILL, RILNET outperforms DRILL in data loss and maximal link delay. Specifically, the maximal link data loss and the maximal link delay of RILNET are 44.4\% and 25.4\% smaller than DRILL, respectively.},
  isbn = {978-3-030-19945-6},
  langid = {english},
  keywords = {Datacenter network,Flowlet,Load balancing,Machine learning,Reinforcement learning},
  file = {C\:\\Users\\lwx1222086\\Zotero\\storage\\HRMPN3NL\\Lin et al_2019_RILNET.pdf}
}

@inbook{inbook,
author = {Lin, Qinliang and Gong, Zhibo and Wang, Qiaoling and Li, Jinlong},
year = {2019},
month = {05},
pages = {44-55},
title = {RILNET: A Reinforcement Learning Based Load Balancing Approach for Datacenter Networks},
isbn = {978-3-030-19944-9},
doi = {10.1007/978-3-030-19945-6_4}
}

@article{kim2021deep,
  title={{Deep Reinforcement Learning Based Active Queue Management For Iot Networks}},
  author={Kim, Minsu and Jaseemuddin, Muhammad and Anpalagan, Alagan},
  journal={Journal of Network and Systems Management},
  volume={29},
  number={3},
  pages={34},
  year={2021},
doi = {},
  publisher={Springer}
}

@inproceedings{mai2020multi,
  title={{Multi-Agent Actor-Critic Reinforcement Learning Based In-network Load Balance}},
  author={Mai, Tianle and Yao, Haipeng and Xiong, Zehui and Guo, Song and Niyato, Dusit Tao},
  booktitle={GLOBECOM 2020-2020 IEEE Global Communications Conference},
  pages={1--6},
  year={2020},
}

@inproceedings{mai2020multi_,
  title={{Multi-Agent Actor-Critic Reinforcement Learning Based In-network Load Balance}},
  author={Mai, Tianle and Yao, Haipeng and Xiong, Zehui and Guo, Song and Niyato, Dusit Tao},
  booktitle={IEEE GLOBECOM},
  pages={1--6},
  year={2020},
}

@inproceedings{fawaz2023graph,
  title={{Graph Convolutional Reinforcement Learning For Load Balancing And Smart Queuing}},
  author={Fawaz, Hassan and Houidi, Omar and Zeghlache, Djamal and Lesca, Julien and Quang, Pham Tran Anh and Leguay, J{\'e}r{\'e}mie and Medagliani, Paolo},
  booktitle={2023 IFIP Networking Conference (IFIP Networking)},
  doi = {10.23919/IFIPNetworking57963.2023.10186430},
  pages={1--9},
  year={2023},
  organization={IEEE}
}

@inproceedings{fawaz2023graph_,
  title={{Graph Convolutional Reinforcement Learning For Load Balancing And Smart Queuing}},
  author={Fawaz, Hassan and Houidi, Omar and Zeghlache, Djamal and Lesca, Julien and Quang, Pham Tran Anh and Leguay, J{\'e}r{\'e}mie and Medagliani, Paolo},
  booktitle={IFIP Networking},
  year={2023},
  organization={IEEE}
}

@inproceedings{houidi2022constrained,
  title={{Constrained Deep Reinforcement Learning For Smart Load Balancing}},
  author={Houidi, Omar and Zeghlache, Djamal and Perrier, Victor and Quang, Pham Tran Anh and Huin, Nicolas and Leguay, J{\'e}r{\'e}mie and Medagliani, Paolo},
  booktitle={2022 IEEE 19th Annual Consumer Communications \& Networking Conference (CCNC)},
  pages={207--215},
doi = {10.1109/CCNC49033.2022.9700657},
  year={2022},
  organization={IEEE}
}

@inproceedings{houidi2022constrained_,
  title={{Constrained Deep Reinforcement Learning For Smart Load Balancing}},
  author={Houidi, Omar and Zeghlache, Djamal and Perrier, Victor and Quang, Pham Tran Anh and Huin, Nicolas and Leguay, J{\'e}r{\'e}mie and Medagliani, Paolo},
  booktitle={IEEE CCNC},
  pages={207--215},
doi = {10.1109/CCNC49033.2022.9700657},
  year={2022},
}

@inproceedings{xu2018experience,
  title={{Experience-driven networking: A Deep Reinforcement Learning Based Approach}},
  author={Xu, Zhiyuan and Tang, Jian and Meng, Jingsong and Zhang, Weiyi and Wang, Yanzhi and Liu, Chi Harold and Yang, Dejun},
  booktitle = {IEEE INFOCOM 2018 - IEEE Conference on Computer Communications},
    pages = {1871–1879},
    numpages = {9},
  year={2018}
}

@inproceedings{xu2018experience_,
  title={{Experience-driven networking: A Deep Reinforcement Learning Based Approach}},
  author={Xu, Zhiyuan and Tang, Jian and Meng, Jingsong and Zhang, Weiyi and Wang, Yanzhi and Liu, Chi Harold and Yang, Dejun},
  booktitle = {IEEE INFOCOM},
    pages = {1871–1879},
    numpages = {9},
  year={2018}
}


@article{benAmeur2006,
 author = {Ben-Ameur, Walid and Ouorou, Adam},
 title = {{Mathematical Models Of The Delay Constrained Routing Problem}},
 journal = {Algorithmic Operations Research},
 volume = {1},
 number = {2},
 year = {2006}
}


@book{kleinrock2007communication,
  title={{Communication Nets: Stochastic Message Flow And Delay}},
  author={Kleinrock, Leonard},
  year={2007},
  publisher={Courier Corporation}
}

@inproceedings{magnouche2021distributeda,
  title={Distributed Utility Maximization From the Edge in IP Networks},
  author={Magnouche, Youcef and Quang, Pham Tran Anh and Leguay, J{\'e}r{\'e}mie and Gong, Xu and Zeng, Feng},
  booktitle={2021 IFIP/IEEE IM}, year={2021}
}
@INPROCEEDINGS{magnouche2021distributed,

  author={Magnouche, Youcef and Quang, Pham Tran Anh and Leguay, Jérémie and Gong, Xu and Zeng, Feng},

  booktitle={2021 IFIP/IEEE International Symposium on Integrated Network Management (IM)}, 

  title={{Distributed Utility Maximization From the Edge in IP Networks}}, 

  year={2021},

  volume={},

  number={},

  pages={224-232},

  doi={}}


@inproceedings{quang2022intent,
  title={{Intent-Based Routing Policy Optimization in SD-WAN}},
  author={Quang, Pham Tran Anh and Martin, Sebastien and Leguay, J{\'e}r{\'e}mie and Gong, Xu and Huiying, Xu},
  booktitle={ICC 2022-IEEE International Conference on Communications},
  pages={4914--4919},
  year={2022},
}

@inproceedings{kamriConstrainedPolicyOptimization2021b,
  title = {Constrained {{Policy Optimization}} for {{Load Balancing}}},
  booktitle = {2021 17th {{International Conference}} on the {{Design}} of {{Reliable Communication Networks}} ({{DRCN}})},
  author = {Kamri, Ahmed Yassine and Quang, Pham Tran Anh and Huin, Nicolas and Leguay, J{\'e}r{\'e}mie},
  year = {2021},
  month = apr,
  pages = {1--6},
  doi = {10.1109/DRCN51631.2021.9477375},
  abstract = {To improve the bandwidth utilization in IP networks, a centralized controller splits flow aggregates over multiple paths and decides load balancing weights. Ideally, load balancing policies should anticipate the impact of their decisions on the Quality of Service (QoS). However, the embedding of accurate performance models into load balancing optimization algorithms is a challenge. In this context, we propose a Deep Reinforcement Learning (DRL) based solution that is able to learn the relationship between traffic and QoS, while providing safety to maximize throughput and avoid violating link capacity constraints. Our safe solution for QoS-aware load balancing integrates DRL algorithms with the Reward Constrained Policy Optimization algorithm. In a scenario where link delays follow the M/M/1 queuing model, we demonstrate, using a non-linear integer program, that our solution can reach a close to optimal end-to-end delay. We also show that our solution automatically learns reward parameters to meet capacity constraints.},
  keywords = {Delays,Load management,Quality of service,Reinforcement learning,Reliability engineering,Safety,Throughput},
  file = {C\:\\Users\\lwx1222086\\Zotero\\storage\\PIRKQ97A\\Kamri et al_2021_Constrained Policy Optimization for Load Balancing.pdf;C\:\\Users\\lwx1222086\\Zotero\\storage\\WCUZLQQG\\stamp.html}
}
@misc{tesslerRewardConstrainedPolicy2018a,
      title={{Reward Constrained Policy Optimization}}, 
      author={Chen Tessler and Daniel J. Mankowitz and Shie Mannor},
      year={2018},
      eprint={1805.11074},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}
@article{tesslerRewardConstrainedPolicy2018,
  author       = {Chen Tessler and
                  Daniel J. Mankowitz and
                  Shie Mannor},
  title        = {{Reward Constrained Policy Optimization}},
  journal      = { Computing Research Repository (CoRR)},
  volume       = {abs/1805.11074},
  year         = {2018},
  eprinttype    = {arXiv},
  eprint       = {1805.11074},
  timestamp    = {Mon, 13 Aug 2018 16:47:13 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/abs-1805-11074.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{troiaDeepReinforcementLearning2021,
  title = {On {{Deep Reinforcement Learning}} for {{Traffic Engineering}} in {{SD-WAN}}},
  author = {Troia, Sebastian and Sapienza, Federico and Var{\'e}, Leonardo and Maier, Guido},
  year = {2021},
  month = jul,
  journal = {IEEE Journal on Selected Areas in Communications},
  volume = {39},
  number = {7},
  pages = {2198--2212},
  issn = {1558-0008},
  doi = {10.1109/JSAC.2020.3041385},
  abstract = {The demand for reliable and efficient Wide Area Networks (WANs) from business customers is continuously increasing. Companies and enterprises use WANs to exchange critical data between headquarters, far-off business branches and cloud data centers. Many WANs solutions have been proposed over the years, such as: leased lines, Frame Relay, Multi-Protocol Label Switching (MPLS), Virtual Private Networks (VPN). Each solution positions differently in the trade-off between reliability, Quality of Service (QoS) and cost. Today, the emerging technology for WAN is Software-Defined Wide Area Networking (SD-WAN) that introduces the Software-Defined Networking (SDN) paradigm into the enterprise-network market. SD-WAN can support differentiated services over public WAN by dynamically reconfiguring in real-time network devices at the edge of the network according to network measurements and service requirements. On the one hand, SD-WAN reduces the high costs of guaranteed QoS WAN solutions (as MPLS), without giving away reliability in practical scenarios. On the other, it brings numerous technical challenges, such as the implementation of Traffic Engineering (TE) methods. TE is critically important for enterprises not only to efficiently orchestrate network traffic among the edge devices, but also to keep their services always available. In this work, we develop different kind of TE algorithms with the aim of improving the performance of an SD-WAN based network in terms of service availability. We first evaluate the performance of baseline TE algorithms. Then, we implement different deep Reinforcement Learning (deep-RL) algorithms to overcome the limitations of the baseline approaches. Specifically, we implement three kinds of deep-RL algorithms, which are: policy gradient, TD- {$\lambda$} and deep Q-learning. Results show that a deep-RL algorithm with a well-designed reward function is capable of increasing the overall network availability and guaranteeing network protection and restoration in SD-WAN.},
  keywords = {Cloud computing,deep reinforcement learning,Enterprise Networking,Multiprotocol label switching,Quality of service,read,Routing,Software-Defined Networking (SDN),Software-Defined Wide Area Network (SD-WAN),Switches,Virtual private networks,Wide area networks},
  file = {C\:\\Users\\lwx1222086\\Zotero\\storage\\CWP96IUM\\Troia et al_2021_On Deep Reinforcement Learning for Traffic Engineering in SD-WAN.pdf}
}

@book{bertsekasDataNetworks1992,
  title = {Data {{Networks}}},
  author = {Bertsekas, Dimitri P. and Gallager, Robert G.},
  year = {1992},
  publisher = {{Prentice Hall}},
  abstract = {Based on an extremely popular short course conducted by the authors for several Fortune 500 companies, this volume is designed to help professionals develop a deeper understanding of data networks and evolving integrated networks, and to explore today's various analysis and design tools. KEY TOPICS:  It begins with an overview of the principles behind data networks, then develops an understanding of the modeling issues and mathematical analysis needed to compare the effectiveness of different networks.   An ideal reference for Communication, Network, and Research and Development Engineers.},
  googlebooks = {i\_lSAAAAMAAJ},
  isbn = {978-0-13-200916-4},
  langid = {english}
}

@article{bouacidaPracticalDynamicBuffer2019,
  title = {Practical and {{Dynamic Buffer Sizing Using LearnQueue}}},
  author = {Bouacida, Nader and Shihada, Basem},
  year = {2019},
  month = aug,
  journal = {IEEE Transactions on Mobile Computing},
  volume = {18},
  number = {8},
  pages = {1885--1897},
  issn = {1558-0660},
  doi = {10.1109/TMC.2018.2868670},
  abstract = {Wireless networks are undergoing an unprecedented revolution in the last decade. With the explosion of delay-sensitive applications usage on the Internet (i.e., online gaming, VoIP, and safety-critical applications), latency becomes a major issue for the development of wireless technology since it has an enormous impact on user experience. In fact, in a phenomenon known as bufferbloat, large static buffers inside the network devices results in increasing the time that packets spend in the queues and, thus, causing larger delays. Concerns have arisen about designing efficient queue management schemes to mitigate the effects of over-buffering in wireless devices. In this paper, we advocate the exploitation of machine learning techniques for dynamic buffer sizing. We propose LearnQueue, a novel reinforcement learning design that can effectively control the latency in wireless networks. LearnQueue adapts quickly and intelligently to changes in the wireless environment using a sophisticated reward structure. The latency control is performed dynamically by tuning the buffer size. Adopting a trial-and-error approach, the proposed scheme penalizes the actions resulting in longer delays or hurting the throughput. In addition, the scheme parameters are designed for an optimized operation depending on different applications requirements. Using the latest generation of WARP hardware, we investigated LearnQueue performance in various network scenarios. The testbed results prove that LearnQueue can grantee low latency while preserving throughput under various congestion situations. We also discuss the feasibility and possible limitations of large-scale deployment of the proposed scheme in wireless devices.},
  keywords = {active queue management,Bufferbloat,Delays,dynamic buffer sizing,Heuristic algorithms,Internet,latency,Learning (artificial intelligence),reinforcement learning,Throughput,wireless networks,Wireless networks},
  file = {C\:\\Users\\lwx1222086\\Zotero\\storage\\DPURISNN\\Bouacida_Shihada_2019_Practical and Dynamic Buffer Sizing Using LearnQueue.pdf}
}

@journal{linRILNETReinforcementLearning2019a,
  title = {{{RILNET}}: {{A Reinforcement Learning Based Load Balancing Approach}} for {{Datacenter Networks}}},
  shorttitle = {{{RILNET}}},
  booktitle = {Machine {{Learning}} for {{Networking}}},
  author = {Lin, Qinliang and Gong, Zhibo and Wang, Qiaoling and Li, Jinlong},
  editor = {Renault, {\'E}ric and M{\"u}hlethaler, Paul and Boumerdassi, Selma},
  year = {2019},
  series = {Lecture {{Notes}} in {{Computer Science}}},
  pages = {44--55},
  publisher = {{Springer International Publishing}},
  address = {{Cham}},
  doi = {10.1007/978-3-030-19945-6_4},
  abstract = {Modern datacenter networks are facing various challenges, e.g., highly dynamic workloads, congestion, topology asymmetry. ECMP, as a traditional load balancing mechanism which is widely used in~today's datacenters, can balance load poorly and lead to congestion. Variety of load balancing schemes are proposed to address the problems of ECMP. However, these traditional schemes usually make load balancing decision only based on network knowledge for a snapshot or a short time past. In this paper, we propose a Reinforcement Learning (RL) based approach, called RILNET (ReInforcement Learning NETworking), aiming at load balancing for datacenter networks. RILNET employs RL to learn a network and control it based on the learned experience. To achieve a higher granularity of control, RILNET is constructed to route flowlet rather than flows. Moreover, RILNET makes routing decisions for aggregation flows (an aggregation flow is a flow set that includes all flows flowing from the same source edge switch to the same destination edge switch) instead of a single flow. In order to test performance of RILNET, we propose a flow-level simulation and a packet-level simulation, and the both results show that RILNET can balance traffic load much more effectively than ECMP and another load balancing solution, i.e., DRILL. Compared with DRILL, RILNET outperforms DRILL in data loss and maximal link delay. Specifically, the maximal link data loss and the maximal link delay of RILNET are 44.4\% and 25.4\% smaller than DRILL, respectively.},
  isbn = {978-3-030-19945-6},
  langid = {english},
  keywords = {Datacenter network,Flowlet,Load balancing,Machine learning,Reinforcement learning},
  file = {C\:\\Users\\lwx1222086\\Zotero\\storage\\HRMPN3NL\\Lin et al_2019_RILNET.pdf}
}

@article{rikhtegarDeepRLBDeepReinforcement2021,
  title = {{{DeepRLB}}: {{A}} Deep Reinforcement Learning-Based Load Balancing in Data Center Networks},
  shorttitle = {{{DeepRLB}}},
  author = {Rikhtegar, Negar and Bushehrian, Omid and Keshtgari, Manijeh},
  year = {2021},
  journal = {International Journal of Communication Systems},
  volume = {34},
  number = {15},
  pages = {e4912},
  issn = {1099-1131},
  doi = {10.1002/dac.4912},
  urldate = {2023-06-26},
  abstract = {Data center networks (DCNs) are facing challenging control problems such as flow scheduling, congestion control, load balancing, and bandwidth allocation when dynamically handling heterogeneous mice and elephant flows. This paper focuses on the load balancing in DCNs as an online decision-making problem with high complexity (NP-hard problem). Traditional load balancing approaches are usually the heuristic algorithms relying on the operator's viewpoint and a short-term knowledge of the traffic conditions and network environment. This paper proposes DeepRLB, a deep reinforcement learning (DRL)-based load balancing approach for software-defined networking-based DCNs which exploits the deep deterministic policy gradient (DDPG) algorithm to adaptively learn the link-weight values by observing the traffic flow characteristics. The actor and critic neural networks in the DDPG model have been designed based on two learning models: fully connected (DeepRLB-Full) and convolutional (DeepRLB-Conv). The output of the model is further used by the controller to determine the forwarding paths for traffic flows accordingly. We evaluated the performance of DeepRLB by comparing it with ECMP as well as a per-packet load balancing algorithm in three different data center topologies under 30 heterogeneous traffic demand matrices. The obtained results showed that the DeepRLB algorithm outperforms the ECMP with respect to studied load balancing metrics considerably (DeepRLB-Conv achieved the best performance). As a sample, DeepRLB-Full and DeepRLB-Conv were able to reach 19.14\% and 24.46\% reduction in the total number of over-utilized and under-utilized network links compared to ECMP, respectively.},
  copyright = {\textcopyright{} 2021 John Wiley \& Sons Ltd.},
  langid = {english},
  keywords = {convolutional neural networks,data center network,deep deterministic policy gradient,deep reinforcement learning,fully connected neural networks,load balancing}
}



@article{DBLP:journals/corr/abs-1903-08792,
  author       = {Richard Cheng and
                  G{\'{a}}bor Orosz and
                  Richard M. Murray and
                  Joel W. Burdick},
  title        = {End-to-End Safe Reinforcement Learning through Barrier Functions for
                  Safety-Critical Continuous Control Tasks},
  journal      = { Computing Research Repository (CoRR)},
  volume       = {abs/1903.08792},
  year         = {2019},
  eprinttype    = {arXiv},
  eprint       = {1903.08792},
  timestamp    = {Mon, 01 Apr 2019 14:07:37 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/abs-1903-08792.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}



@article{chengEndtoEndSafeReinforcement2019,
  title = {End-to-{{End Safe Reinforcement Learning}} through {{Barrier Functions}} for {{Safety-Critical Continuous Control Tasks}}},
  author = {Cheng, Richard and Orosz, Gabor and Murray, Richard M. and Burdick, Joel W.},
  year = {2019},
  month = mar,
  number = {arXiv:1903.08792},
  journal      = {Computing Research Repository (CoRR)},
  volume       = {abs/1903.08792},
  eprint = {1903.08792},
  primaryclass = {cs, stat},
  publisher = {{arXiv}},
  urldate = {2022-12-19},
  abstract = {Reinforcement Learning (RL) algorithms have found limited success beyond simulated applications, and one main reason is the absence of safety guarantees during the learning process. Real world systems would realistically fail or break before an optimal controller can be learned. To address this issue, we propose a controller architecture that combines (1) a model-free RL-based controller with (2) model-based controllers utilizing control barrier functions (CBFs) and (3) on-line learning of the unknown system dynamics, in order to ensure safety during learning. Our general framework leverages the success of RL algorithms to learn high-performance controllers, while the CBF-based controllers both guarantee safety and guide the learning process by constraining the set of explorable polices. We utilize Gaussian Processes (GPs) to model the system dynamics and its uncertainties. Our novel controller synthesis algorithm, RL-CBF, guarantees safety with high probability during the learning process, regardless of the RL algorithm used, and demonstrates greater policy exploration efficiency. We test our algorithm on (1) control of an inverted pendulum and (2) autonomous car-following with wireless vehicle-to-vehicle communication, and show that our algorithm attains much greater sample efficiency in learning than other state-of-the-art algorithms and maintains safety during the entire learning process.},
  archiveprefix = {arxiv},
  keywords = {Computer Science - Machine Learning,Electrical Engineering and Systems Science - Systems and Control,favorite,interesting,Statistics - Machine Learning},
  file = {C\:\\Users\\lwx1222086\\Zotero\\storage\\EJZEABZI\\Cheng et al_2019_End-to-End Safe Reinforcement Learning through Barrier Functions for.pdf;C\:\\Users\\lwx1222086\\Zotero\\storage\\2DYSK5MP\\1903.html}
}

@article{bestuzhevaSCIPOptimizationSuite2021,
  title = {The {{SCIP Optimization Suite}} 8.0},
  author = {Bestuzheva, Ksenia and Besan{\c c}on, Mathieu and et al.},
  year = {2021},
  month = dec,
  number = {arXiv:2112.08872},
  eprint = {2112.08872},
  primaryclass = {math},
  publisher = {{arXiv}},
  journal      = {Computing Research Repository (CoRR)},
  volume       = {abs/2112.08872},
  doi = {10.48550/arXiv.2112.08872},
  urldate = {2023-07-01},
  abstract = {The SCIP Optimization Suite provides a collection of software packages for mathematical optimization centered around the constraint integer programming framework SCIP. This paper discusses enhancements and extensions contained in version 8.0 of the SCIP Optimization Suite. Major updates in SCIP include improvements in symmetry handling and decomposition algorithms, new cutting planes, a new plugin type for cut selection, and a complete rework of the way nonlinear constraints are handled. Additionally, SCIP 8.0 now supports interfaces for Julia as well as Matlab. Further, UG now includes a unified framework to parallelize all solvers, a utility to analyze computational experiments has been added to GCG, dual solutions can be postsolved by PaPILO, new heuristics and presolving methods were added to SCIP-SDP, and additional problem classes and major performance improvements are available in SCIP-Jack.},
  archiveprefix = {arxiv},
  keywords = {{90C05, 90C10, 90C11, 90C30, 90C90, 65Y05},Mathematics - Optimization and Control},
  file = {C\:\\Users\\lwx1222086\\Zotero\\storage\\FAU9DING\\Bestuzheva et al_2021_The SCIP Optimization Suite 8.pdf}
}

@article{schulmanProximalPolicyOptimization2017,
  abstract = {We propose a new family of policy gradient methods for reinforcement learning, which alternate between sampling data through interaction with the environment, and optimizing a "surrogate" objective function using stochastic gradient ascent. Whereas standard policy gradient methods perform one gradient update per data sample, we propose a novel objective function that enables multiple epochs of minibatch updates. The new methods, which we call proximal policy optimization (PPO), have some of the benefits of trust region policy optimization (TRPO), but they are much simpler to implement, more general, and have better sample complexity (empirically). Our experiments test PPO on a collection of benchmark tasks, including simulated robotic locomotion and Atari game playing, and we show that PPO outperforms other online policy gradient methods, and overall strikes a favorable balance between sample complexity, simplicity, and wall-time. },
  added-at = {2019-12-16T18:31:56.000+0100},
  
  author = {Schulman, John and Wolski, Filip and Dhariwal, Prafulla and Radford, Alec and Klimov, Oleg},
  biburl = {https://www.bibsonomy.org/bibtex/24bbcce6aa1c42ae7f61ef8cf5475aa85/lanteunis},
  ee = {http://arxiv.org/abs/1707.06347},
  interhash = {f57ff463a90dbafb77d55a25aea8355c},
  intrahash = {4bbcce6aa1c42ae7f61ef8cf5475aa85},
  journal = { Computing Research Repository (CoRR)},
number = {arXiv:1707.06347},
  keywords = {DRLAlgoComparison ppo reinforcement_learning},
  timestamp = {2019-12-18T21:15:59.000+0100},
  title = {Proximal Policy Optimization Algorithms.},
  volume = {abs/1707.06347},
  
  year = 2017
}



@article{schulmanProximalPolicyOptimization2017a,
  title = {Proximal {{Policy Optimization Algorithms}}},
  author = {Schulman, John and Wolski, Filip and Dhariwal, Prafulla and Radford, Alec and Klimov, Oleg},
  year = {2017},
  month = aug,
  number = {arXiv:1707.06347},
  eprint = {1707.06347},
  primaryclass = {cs},
  publisher = {{arXiv}},
  urldate = {2023-01-27},
  abstract = {We propose a new family of policy gradient methods for reinforcement learning, which alternate between sampling data through interaction with the environment, and optimizing a ``surrogate'' objective function using stochastic gradient ascent. Whereas standard policy gradient methods perform one gradient update per data sample, we propose a novel objective function that enables multiple epochs of minibatch updates. The new methods, which we call proximal policy optimization (PPO), have some of the benefits of trust region policy optimization (TRPO), but they are much simpler to implement, more general, and have better sample complexity (empirically). Our experiments test PPO on a collection of benchmark tasks, including simulated robotic locomotion and Atari game playing, and we show that PPO outperforms other online policy gradient methods, and overall strikes a favorable balance between sample complexity, simplicity, and wall-time.},
  archiveprefix = {arxiv},
  langid = {english},
  keywords = {Computer Science - Machine Learning},
  file = {C\:\\Users\\lwx1222086\\Zotero\\storage\\HMMGWB6Y\\Schulman et al. - 2017 - Proximal Policy Optimization Algorithms.pdf}
}


@article{lillicrapContinuousControlDeep2019,
  title = {{Continuous Control With Deep Reinforcement Learning}},
  author = {Lillicrap, Timothy P. and Hunt, Jonathan J. and Pritzel, Alexander and Heess, Nicolas and Erez, Tom and Tassa, Yuval and Silver, David and Wierstra, Daan},
  year = {2019},
  month = jul,
  number = {arXiv:1509.02971},
  eprint = {1509.02971},
  journal      = {Computing Research Repository (CoRR)},
  volume       = {abs/1509.02971},
  primaryclass = {cs, stat},
  publisher = {{arXiv}},
  urldate = {2023-01-27},
  abstract = {We adapt the ideas underlying the success of Deep Q-Learning to the continuous action domain. We present an actor-critic, model-free algorithm based on the deterministic policy gradient that can operate over continuous action spaces. Using the same learning algorithm, network architecture and hyper-parameters, our algorithm robustly solves more than 20 simulated physics tasks, including classic problems such as cartpole swing-up, dexterous manipulation, legged locomotion and car driving. Our algorithm is able to find policies whose performance is competitive with those found by a planning algorithm with full access to the dynamics of the domain and its derivatives. We further demonstrate that for many of the tasks the algorithm can learn policies ``end-to-end'': directly from raw pixel inputs.},
  archiveprefix = {arxiv},
  langid = {english},
  keywords = {Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {C\:\\Users\\lwx1222086\\Zotero\\storage\\IWZ27Y9H\\Lillicrap et al. - 2019 - Continuous control with deep reinforcement learnin.pdf}
}

@inproceedings{silverDeterministicPolicyGradient2014,
  title = {{Deterministic Policy Gradient Algorithms}},
  booktitle = {Proceedings of the 31st {{International Conference}} on {{International Conference}} on {{Machine Learning}} - {{Volume}} 32},
  author = {Silver, David and Lever, Guy and Heess, Nicolas and Degris, Thomas and Wierstra, Daan and Riedmiller, Martin},
  year = {2014},
  month = jun,
  series = {{{ICML}}'14},
  pages = {I-387--I-395},
  publisher = {{JMLR.org}},
  address = {{Beijing, China}},
  urldate = {2023-07-04},
doi = {10.5555/3044805.3044850},
  abstract = {In this paper we consider deterministic policy gradient algorithms for reinforcement learning with continuous actions. The deterministic policy gradient has a particularly appealing form: it is the expected gradient of the action-value function. This simple form means that the deterministic policy gradient can be estimated much more efficiently than the usual stochastic policy gradient. To ensure adequate exploration, we introduce an off-policy actor-critic algorithm that learns a deterministic target policy from an exploratory behaviour policy. We demonstrate that deterministic policy gradient algorithms can significantly outperform their stochastic counterparts in high-dimensional action spaces.}
}

@inproceedings{silverDeterministicPolicyGradient2014_,
  title = {{Deterministic Policy Gradient Algorithms}},
  booktitle = {ICML},
  author = {Silver, David and Lever, Guy and Heess, Nicolas and Degris, Thomas and Wierstra, Daan and Riedmiller, Martin},
  year = {2014},
  month = jun,
  pages = {I-387--I-395},
  urldate = {2023-07-04},
}


@article{andrychowiczHindsightExperienceReplay2018,
  author       = {Marcin Andrychowicz and
                  Filip Wolski and
                  Alex Ray and
                  Jonas Schneider and
                  Rachel Fong and
                  Peter Welinder and
                  Bob McGrew and
                  Josh Tobin and
                  Pieter Abbeel and
                  Wojciech Zaremba},
  title        = {{Hindsight Experience Replay}},
  journal      = { Computing Research Repository (CoRR)},
  volume       = {abs/1707.01495},
  year         = {2017},
  eprinttype    = {arXiv},
  eprint       = {1707.01495},
  timestamp    = {Fri, 08 Nov 2019 12:51:04 +0100},
  biburl       = {https://dblp.org/rec/journals/corr/AndrychowiczWRS17.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{andrychowiczHindsightExperienceReplay2018a,
  title = {Hindsight {{Experience Replay}}},
  author = {Andrychowicz, Marcin and Wolski, Filip and Ray, Alex and Schneider, Jonas and Fong, Rachel and Welinder, Peter and McGrew, Bob and Tobin, Josh and Abbeel, Pieter and Zaremba, Wojciech},
  year = {2018},
  month = feb,
  number = {arXiv:1707.01495},
  eprint = {1707.01495},
  primaryclass = {cs},
  publisher = {{arXiv}},
  urldate = {2023-07-04},
  abstract = {Dealing with sparse rewards is one of the biggest challenges in Reinforcement Learning (RL). We present a novel technique called Hindsight Experience Replay which allows sample-efficient learning from rewards which are sparse and binary and therefore avoid the need for complicated reward engineering. It can be combined with an arbitrary off-policy RL algorithm and may be seen as a form of implicit curriculum. We demonstrate our approach on the task of manipulating objects with a robotic arm. In particular, we run experiments on three different tasks: pushing, sliding, and pick-and-place, in each case using only binary rewards indicating whether or not the task is completed. Our ablation studies show that Hindsight Experience Replay is a crucial ingredient which makes training possible in these challenging environments. We show that our policies trained on a physics simulation can be deployed on a physical robot and successfully complete the task.},
  archiveprefix = {arxiv},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Machine Learning,Computer Science - Neural and Evolutionary Computing,Computer Science - Robotics},
  file = {C\:\\Users\\lwx1222086\\Zotero\\storage\\VHZLEHIR\\Andrychowicz et al_2018_Hindsight Experience Replay.pdf;C\:\\Users\\lwx1222086\\Zotero\\storage\\LPB5NYMS\\1707.html}
}

@article{Kullback51klDivergencea,
  added-at = {2010-10-31T19:59:47.000+0100},
  author = {Kullback, S. and Leibler, R. A.},
  biburl = {https://www.bibsonomy.org/bibtex/2560a5719c537c5c4a496bfebd4a21603/lee_peck},
  description = {Kullback , Leibler : On Information and Sufficiency},
  interhash = {f9d41d76a07383cca4c3a1a94c24d533},
  intrahash = {560a5719c537c5c4a496bfebd4a21603},
  journal = {Ann. Math. Statist.},
  keywords = {51 Kullback Leibler divergence kl},
  number = 1,
  pages = {79-86},
  timestamp = {2010-10-31T19:59:47.000+0100},
  doi = {10.1214/aoms/1177729694},
  title = {{On Information And Sufficiency}},
  volume = 22,
  year = 1951
}
@article{Kullback51klDivergence,
 ISSN = {00034851},
 author = {S. Kullback and R. A. Leibler},
 journal = {The Annals of Mathematical Statistics},
 number = {1},
 pages = {79--86},
 publisher = {Institute of Mathematical Statistics},
 title = {On Information and Sufficiency},
 doi = {10.1214/aoms/1177729694},
 urldate = {2023-09-15},
 volume = {22},
 year = {1951}
}


@misc{openaigyma,
  Author = {Greg Brockman and Vicki Cheung and Ludwig Pettersson and Jonas Schneider and John Schulman and Jie Tang and Wojciech Zaremba},
  Title = {OpenAI Gym},
  Year = {2016},
  Eprint = {arXiv:1606.01540},
}
@misc{openaigymc,
      title={OpenAI Gym}, 
      author={Greg Brockman and Vicki Cheung and Ludwig Pettersson and Jonas Schneider and John Schulman and Jie Tang and Wojciech Zaremba},
      year={2016},
      name={1606.01540},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@article{openaigym,
  title={{OpenAI Gym}},
  author={Greg Brockman and Vicki Cheung and Ludwig Pettersson and Jonas Schneider and John Schulman and Jie Tang and Wojciech Zaremba},
  journal={ArXiv},
  year={2016},
  volume={abs/1606.01540},
}

@misc{openaigymb,
  title = {{{OpenAI Gym}}},
  author = {Brockman, Greg and Cheung, Vicki and Pettersson, Ludwig and Schneider, Jonas and Schulman, John and Tang, Jie and Zaremba, Wojciech},
  year = {2016},
  month = jun,
  number = {arXiv:1606.01540},
  eprint = {1606.01540},
  primaryclass = {cs},
  publisher = {{arXiv}},
  doi = {10.48550/arXiv.1606.01540},
  urldate = {2023-09-14},
  abstract = {OpenAI Gym is a toolkit for reinforcement learning research. It includes a growing collection of benchmark problems that expose a common interface, and a website where people can share their results and compare the performance of algorithms. This whitepaper discusses the components of OpenAI Gym and the design decisions that went into the software.},
  archiveprefix = {arxiv},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Machine Learning},
  file = {C\:\\Users\\lwx1222086\\Zotero\\storage\\RY5ZTETL\\Brockman et al_2016_OpenAI Gym.pdf}
}


@inproceedings{yang2019softwarea,
  title={{Software-defined wide area network (SD-WAN): Architecture, advances and opportunities}},
  author={Yang, Zhenjie and Cui, Yong and Li, Baochun and Liu, Yadong and Xu, Yi},
  booktitle={Proc. IEEE ICCCN},
  year={2019}
}
@INPROCEEDINGS{yang2019software,

  author={Yang, Zhenjie and Cui, Yong and Li, Baochun and Liu, Yadong and Xu, Yi},

  booktitle={2019 28th International Conference on Computer Communication and Networks (ICCCN)}, 

  title={{Software-Defined Wide Area Network (SD-WAN): Architecture, Advances and Opportunities}}, 

  year={2019},

  volume={},

  number={},

  pages={1-9},

  doi={10.1109/ICCCN.2019.8847124}}

@INPROCEEDINGS{yang2019software_,

  author={Yang, Zhenjie and Cui, Yong and Li, Baochun and Liu, Yadong and Xu, Yi},

  booktitle={IEEE ICCCN}, 

  title={{Software-Defined Wide Area Network (SD-WAN): Architecture, Advances and Opportunities}}, 

  year={2019},

  volume={},

  number={},

  pages={1-9},

  doi={10.1109/ICCCN.2019.8847124}}


@inproceedings{rhamdaniEqualCostMultipathRouting2018,
  title = {Equal-{{Cost Multipath Routing}} in {{Data Center Network Based}} on {{Software Defined Network}}},
  booktitle = {2018 6th {{International Conference}} on {{Information}} and {{Communication Technology}} ({{ICoICT}})},
  author = {Rhamdani, Fiqih and Suwastika, Novian Anggis and Nugroho, Muhammad Arief},
  year = {2018},
  month = may,
  pages = {222--226},
  abstract = {In Data Center facilities, network performance is crucial. The system performance requirements are usually high throughput and packet loss sensitive. In addition, the data center also requires redundant links, in order to avoid the occurrence of failure in the network. Applying topologies such as as fat-tree can solve the redundant link needs problem. However, the use of redundant links that are only used as backups are considered ineffective. A routing mechanism that can exploit the potential of existing links sufficiently is required. Equal-cost multipath routing (ECMP) is a routing scheme that can be implemented to solve the problem. With the implementation of software defined network (SDN) on the network, the construction of this routing scheme will be more accessible. The ECMP scheme utilizes modified Dijkstra's algorithm to search for the shortest path, and uses the modulo-n hashing method in the selection of the delivery path. This paper implements ECMP scheme on fat-tree topology with SDN-based network. The results obtained in this study prove that the network implementing ECMP can provide a throughput difference of 60.14Mbps when compared with static routing in a 20Mbps bandwidth traffic test scenario. Also the ECMP network can provide 15.72\% less packet loss compared to static routing networks.},
  keywords = {Data centers,Dijkstra,Equal-Cost Multipath,Network topology,Packet loss,Routing,Software Defined Network,Throughput,Topology}
}

@article{alizadehCONGADistributedCongestionaware2014,
  title = {{{CONGA}}: Distributed Congestion-Aware Load Balancing for Datacenters},
  shorttitle = {{{CONGA}}},
  author = {Alizadeh, Mohammad and Edsall, Tom and Dharmapurikar, Sarang and Vaidyanathan, Ramanan and Chu, Kevin and Fingerhut, Andy and Lam, Vinh The and Matus, Francis and Pan, Rong and Yadav, Navindra and Varghese, George},
  year = {2014},
  month = aug,
  journal = {ACM SIGCOMM Computer Communication Review},
  volume = {44},
  number = {4},
  pages = {503--514},
  issn = {0146-4833},
  urldate = {2023-07-07},
  abstract = {We present the design, implementation, and evaluation of CONGA, a network-based distributed congestion-aware load balancing mechanism for datacenters. CONGA exploits recent trends including the use of regular Clos topologies and overlays for network virtualization. It splits TCP flows into flowlets, estimates real-time congestion on fabric paths, and allocates flowlets to paths based on feedback from remote switches. This enables CONGA to efficiently balance load and seamlessly handle asymmetry, without requiring any TCP modifications. CONGA has been implemented in custom ASICs as part of a new datacenter fabric. In testbed experiments, CONGA has 5x better flow completion times than ECMP even with a single link failure and achieves 2-8x better throughput than MPTCP in Incast scenarios. Further, the Price of Anarchy for CONGA is provably small in Leaf-Spine topologies; hence CONGA is nearly as effective as a centralized scheduler while being able to react to congestion in microseconds. Our main thesis is that datacenter fabric load balancing is best done in the network, and requires global schemes such as CONGA to handle asymmetry.},
  keywords = {datacenter fabric,distributed,load balancing}
}

@INPROCEEDINGS{zhangPathPlanningModel2022,

  author={Zhang, Xinyi and Xu, Yunwen and Chen, Youren and Li, Dewei},

  booktitle={2022 41st Chinese Control Conference (CCC)}, 

  title={{Path Planning Model Based on Constrained Policy Iteration}}, 

  year={2022},

  volume={},

  number={},

  pages={5518-5523},

  doi={10.23919/CCC55666.2022.9902612}}


@inproceedings{medagliani2016global,
  title={Global optimization for hash-based splitting},
  author={Medagliani, Paolo and Leguay, Jeremie and Abdullah, Mohammed and Leconte, Mathieu and Paris, Stefano},
doi= {10.1109/GLOCOM.2016.7841861},
  booktitle={Proc. IEEE Global Communications Conference (GLOBECOM)},
  pages={1-6},


  year={2016}
}

@inproceedings{zhou2014wcmp,
  title={WCMP: Weighted cost multipathing for improved fairness in data centers},
  author={Zhou, Junlan and Tewari, Malveeka and Zhu, Min and Kabbani, Abdul and Poutievski, Leon and Singh, Arjun and Vahdat, Amin},
  booktitle={Proceedings of the Ninth European Conference on Computer Systems},
  pages={1--14},
  year={2014}
}

@inproceedings{zhangPathPlanningModel2022a,
  title = {Path {{Planning Model Based}} on {{Constrained Policy Iteration}}},
  booktitle = {2022 41st {{Chinese Control Conference}} ({{CCC}})},
  author = {Zhang, Xinyi and Xu, Yunwen and Chen, Youren and Li, Dewei},
  year = {2022},
  month = jul,
  pages = {5518--5523},
  issn = {1934-1768},
  doi = {10.23919/CCC55666.2022.9902612},
  abstract = {With the increasing severity of traffic congestion, the frequency of traffic emergencies has also increased. When an emergency occurs, it is necessary to send a large number of emergency vehicles from all over the city to the rescue point, therefore, it is necessary to plan the best feasible path from multiple locations to the same destination quickly and efficiently. At the same time, emergencies have a serious impact on urban operation. The emergency management of urban traffic puts forward more and more specific conditions and requirements around path planning: for example, find the path with as few intersections as possible, and find multiple paths with repetition rate constraints. Because the existing intelligent algorithms such as Dijkstra algorithm and PSO algorithm can only find one optimal path from the starting point to the target point, and the unconstrained reinforcement learning algorithm can find multiple paths with poor performance and can not meet the specific traffic display requirements, this paper proposes a model based on constrained policy optimization to solve the path optimization problem in the context of traffic emergency. The model is a continuation of the policy iteration algorithm. When the policy is improved, the action is constrained, and the policy with the largest cumulative reward under the constraints is selected. It can solve multiple paths from the starting point to the target point, and find the path that meets the step constraint and the repetition rate constraint with the known path. When solving the problem of finding the path from multiple points to the target point, the time efficiency is higher than Dijkstra algorithm.},
  keywords = {Aerospace electronics,Constrained Policy Iteration,Emergency services,Excavation,Optimization,Path planning,Path Planning,Reinforcement learning,Reinforcement Learning,Traffic Emergency,Urban areas},
  file = {C\:\\Users\\lwx1222086\\Zotero\\storage\\L3RYMRGK\\Zhang et al_2022_Path Planning Model Based on Constrained Policy Iteration.pdf}
}

@article{amesControlBarrierFunctions2019,
  author       = {Aaron D. Ames and
                  Samuel Coogan and
                  Magnus Egerstedt and
                  Gennaro Notomista and
                  Koushil Sreenath and
                  Paulo Tabuada},
  title        = {{Control Barrier Functions: Theory And Applications}},
  journal      = { Computing Research Repository (CoRR)},
  volume       = {abs/1903.11199},
  year         = {2019},
  eprinttype    = {arXiv},
  eprint       = {1903.11199},
  timestamp    = {Fri, 09 Apr 2021 20:34:31 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/abs-1903-11199.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@misc{amesControlBarrierFunctions2019a,
  title = {Control {{Barrier Functions}}: {{Theory}} and {{Applications}}},
  shorttitle = {Control {{Barrier Functions}}},
  author = {Ames, Aaron D. and Coogan, Samuel and Egerstedt, Magnus and Notomista, Gennaro and Sreenath, Koushil and Tabuada, Paulo},
  year = {2019},
  month = mar,
  number = {arXiv:1903.11199},
  eprint = {1903.11199},
  primaryclass = {cs},
  publisher = {{arXiv}},
  doi = {10.48550/arXiv.1903.11199},
  urldate = {2023-02-06},
  abstract = {This paper provides an introduction and overview of recent work on control barrier functions and their use to verify and enforce safety properties in the context of (optimization based) safety-critical controllers. We survey the main technical results and discuss applications to several domains including robotic systems.},
  archiveprefix = {arxiv},
  keywords = {Electrical Engineering and Systems Science - Systems and Control},
  file = {C\:\\Users\\lwx1222086\\Zotero\\storage\\7IF2VG3J\\Ames et al_2019_Control Barrier Functions.pdf;C\:\\Users\\lwx1222086\\Zotero\\storage\\W8T72JY8\\1903.html}
}

@Inbook{ns3,
author="Riley, George F.
and Henderson, Thomas R.",
title="The ns-3 Network Simulator",
bookTitle="Modeling and Tools for Network Simulation",
year="2010",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages={15--34},
chapter={1},
abstract="As networks of computing devices grow larger and more complex, the need for highly accurate and scalable network simulation technologies becomes critical. Despite the emergence of large-scale testbeds for network research, simulation still plays a vital role in terms of scalability (both in size and in experimental speed), reproducibility, rapid prototyping, and education. With simulation based studies, the approach can be studied in detail at varying scales, with varying data applications, varying field conditions, and will result in reproducible and analyzable results.",
isbn="978-3-642-12331-3",
doi="10.1007/978-3-642-12331-3_2",
}

@article{stable-baselines3,
  author  = {Antonin Raffin and Ashley Hill and Adam Gleave and Anssi Kanervisto and Maximilian Ernestus and Noah Dormann},
  title   = {{Stable-Baselines3: Reliable Reinforcement Learning Implementations}},
  journal = {Journal of Machine Learning Research},
  year    = {2021},
  volume  = {22},
  number  = {268},
  pages   = {1-8},
}

@article{knightInternetTopologyZoo2011,
  title = {The {{Internet Topology Zoo}}},
  author = {Knight, Simon and Nguyen, Hung X. and Falkner, Nickolas and Bowden, Rhys and Roughan, Matthew},
  year = {2011},
  month = oct,
  journal = {IEEE Journal on Selected Areas in Communications},
  volume = {29},
  number = {9},
  pages = {1765--1775},
  issn = {0733-8716},
  doi = {10.1109/JSAC.2011.111002},
  urldate = {2024-01-31},
  abstract = {The study of network topology has attracted a great deal of attention in the last decade, but has been hampered by a lack of accurate data. Existing methods for measuring topology have flaws, and arguments about the importance of these have overshadowed the more interesting questions about network structure. The Internet Topology Zoo is a store of network data created from the information that network operators make public. As such it is the most accurate large-scale collection of network topologies available, and includes meta-data that couldn't have been measured. With this data we can answer questions about network structure with more certainty than ever before {\textemdash} we illustrate its power through a preliminary analysis of the PoP-level topology of over 140 networks. We find a wide range of network designs not conforming as a whole to any obvious model.},
  langid = {english},
  file = {C:\Users\lwx1222086\Zotero\storage\BP52KCDE\Knight et al. - 2011 - The Internet Topology Zoo.pdf}
}

@incollection{Riley2010,
  title = {The Ns-3 Network Simulator},
  booktitle = {Modeling and Tools for Network Simulation},
  author = {Riley, George F. and Henderson, Thomas R.},
  editor = {Wehrle, Klaus and G{\"u}ne{\c s}, Mesut and Gross, James},
  year = {2010},
  pages = {15--34},
  publisher = {Springer Berlin Heidelberg},
  address = {Berlin, Heidelberg},
  doi = {10.1007/978-3-642-12331-3_2},
  abstract = {As networks of computing devices grow larger and more complex, the need for highly accurate and scalable network simulation technologies becomes critical. Despite the emergence of large-scale testbeds for network research, simulation still plays a vital role in terms of scalability (both in size and in experimental speed), reproducibility, rapid prototyping, and education. With simulation based studies, the approach can be studied in detail at varying scales, with varying data applications, varying field conditions, and will result in reproducible and analyzable results.},
  isbn = {978-3-642-12331-3},
  file = {C:\Users\lwx1222086\Zotero\storage\TDGG3I7R\Riley_Henderson_2010_The ns-3 network simulator.pdf}
}

@inproceedings{chavesOFSwitch13EnhancingNs32016,
  title = {{{OFSwitch13}}: {{Enhancing}} Ns-3 with {{OpenFlow}} 1.3 {{Support}}},
  shorttitle = {{{OFSwitch13}}},
  booktitle = {Proceedings of the {{Workshop}} on Ns-3 - {{WNS3}} '16},
  author = {Chaves, Luciano Jerez and Garcia, Islene Calciolari and Madeira, Edmundo Roberto Mauro},
  year = {2016},
  pages = {33--40},
  publisher = {ACM Press},
  address = {Seattle, WA, USA},
  doi = {10.1145/2915371.2915381},
  urldate = {2023-08-02},
  abstract = {The world is witnessing the rapid evolution of communication technologies, and meeting current market requirements is virtually impossible with traditional network architectures. Many works point to the use of Software Defined Networking (SDN) paradigm and the OpenFlow protocol as enabling solutions to overcome current limitations. Despite the fact that the Network Simulator 3 (ns-3 ) already has a module that supports OpenFlow simulations, it is possible to note that the available implementation provides a very outdated protocol version (0.8.9). As many new major features were introduced up to the latest versions, it is interesting to have some of them available for use. In this context, this paper presents the OFSwitch13: a module to enhance the ns-3 with OpenFlow 1.3 technology support. This module provides both an OpenFlow 1.3 switch device and a controller application interface. Details about module design and implementation are discussed throughout this paper, and a case study scenario is used to illustrate some of the available OFSwitch13 module features.},
  isbn = {978-1-4503-4216-2},
  langid = {english},
  file = {C:\Users\lwx1222086\Zotero\storage\DD7CG2TE\Chaves et al. - 2016 - OFSwitch13 Enhancing ns-3 with OpenFlow 1.3 Suppo.pdf}
}

@misc{openflow1_3,
  added-at = {2014-12-10T16:12:02.000+0100},
  author = {{The Open Networking Foundation}},
  biburl = {https://www.bibsonomy.org/bibtex/28f52a475d2a96fc18547db19dca1837b/chesteve},
  interhash = {e4c74255933750c1943f70020c677a91},
  intrahash = {8f52a475d2a96fc18547db19dca1837b},
  keywords = {imported},
  month = {Jun.},
  timestamp = {2014-12-10T16:12:02.000+0100},
  title = {{OpenFlow Switch Specification v1.3.0}},
  xnote = {\url{https://www.opennetworking.org/images/stories/downloads/specification/openflow-spec-v1.3.0.pdf}},
  year = 2012
}



@inproceedings{dinh2024safe,
  title = {{Towards Safe Load Balancing based on Control Barrier Functions and Deep Reinforcement Learning}},
  shorttitle = {Safe Load-Balancing},
  booktitle = {{{IEEE/IFIP Network Operations}} and {{Management Symposium}}},
  author = {Dinh, Lam and Pham, Tran Anh Quang and Leguay, J{\'e}r{\'e}mie},
  year = {2024},
  month = may,
  pages = {1--9},
  publisher = {IEEE},
  eprinttype    = {arXiv},
  eprint       = {2401.05525},
  address = {Seoul, South Korea},
  urldate = {2024-05-23},
  langid = {english},
}


@inproceedings{rhamdaniEqualCostMultipathRouting2018a,
  title = {Equal-{{Cost Multipath Routing}} in {{Data Center Network Based}} on {{Software Defined Network}}},
  booktitle = {2018 6th {{International Conference}} on {{Information}} and {{Communication Technology}} ({{ICoICT}})},
  author = {Rhamdani, Fiqih and Suwastika, Novian Anggis and Nugroho, Muhammad Arief},
  year = {2018},
  month = may,
  pages = {222--226},
  doi = {10.1109/ICoICT.2018.8528730},
  urldate = {2024-04-17},
  abstract = {In Data Center facilities, network performance is crucial. The system performance requirements are usually high throughput and packet loss sensitive. In addition, the data center also requires redundant links, in order to avoid the occurrence of failure in the network. Applying topologies such as as fat-tree can solve the redundant link needs problem. However, the use of redundant links that are only used as backups are considered ineffective. A routing mechanism that can exploit the potential of existing links sufficiently is required. Equal-cost multipath routing (ECMP) is a routing scheme that can be implemented to solve the problem. With the implementation of software defined network (SDN) on the network, the construction of this routing scheme will be more accessible. The ECMP scheme utilizes modified Dijkstra's algorithm to search for the shortest path, and uses the modulo-n hashing method in the selection of the delivery path. This paper implements ECMP scheme on fat-tree topology with SDN-based network. The results obtained in this study prove that the network implementing ECMP can provide a throughput difference of 60.14Mbps when compared with static routing in a 20Mbps bandwidth traffic test scenario. Also the ECMP network can provide 15.72\% less packet loss compared to static routing networks.},
  keywords = {Data centers,Dijkstra,Equal-Cost Multipath,Network topology,Packet loss,Routing,Software Defined Network,Throughput,Topology},
  file = {C:\Users\lwx1222086\Zotero\storage\TP757M3T\Rhamdani et al_2018_Equal-Cost Multipath Routing in Data Center Network Based on Software Defined.pdf}
}

@misc{ASR9000XRUnderstanding2013,
  title = {{{ASR9000}}/{{XR}}: {{Understanding Unequal}} Cost {{Multipath}} ({{UCMP}}), {{DMZ}} Link Bandwidth and Routes},
  author={Cisco},
  shorttitle = {{{ASR9000}}/{{XR}}},
  year = {2013},
  month = apr,
  urldate = {2024-04-17},
  abstract = {Introduction Equal vs Non-Equal cost multipath DMZ link bandwidth Restriction Example using UCMP and DMZ link bandwidth  Topology Configuration Show commands and explanations  show bgp summary (to view the neighbor status) show bgp (to view the received and advertised prefixes) show bgp {$<$}prefix{$>$} (To...},
  chapter = {Service Providers Knowledge Base},
  url = {https://community.cisco.com/t5/service-providers-knowledge-base/asr9000-xr-understanding-unequal-cost-multipath-ucmp-dmz-link/ta-p/3138853},
  langid = {english}
}

@article{brakmoTCPVegasEnd1995,
  title = {{{TCP Vegas}}: End to End Congestion Avoidance on a Global {{Internet}}},
  shorttitle = {{{TCP Vegas}}},
  author = {Brakmo, L.S. and Peterson, L.L.},
  year = {1995},
  month = oct,
  journal = {IEEE Journal on Selected Areas in Communications},
  volume = {13},
  number = {8},
  pages = {1465--1480},
  issn = {1558-0008},
  doi = {10.1109/49.464716},
  urldate = {2024-04-19},
  abstract = {Vegas is an implementation of TCP that achieves between 37 and 71\% better throughput on the Internet, with one-fifth to one-half the losses, as compared to the implementation of TCP in the Reno distribution of BSD Unix. This paper motivates and describes the three key techniques employed by Vegas, and presents the results of a comprehensive experimental performance study, using both simulations and measurements on the Internet, of the Vegas and Reno implementations of TCP.{$<>$}},
  keywords = {Adaptive control,Bandwidth,Computer science,Internet,Jacobian matrices,Programmable control,Protocols,TCPIP,Testing,Throughput}
}

@article{wangNewTrafficPrediction2021,
  title = {A {{New Traffic Prediction Algorithm}} to {{Software Defined Networking}}},
  author = {Wang, Yuqing and Jiang, Dingde and Huo, Liuwei and Zhao, Yong},
  year = {2021},
  month = apr,
  journal = {Mobile Networks and Applications},
  volume = {26},
  number = {2},
  pages = {716--725},
  issn = {1572-8153},
  doi = {10.1007/s11036-019-01423-3},
  urldate = {2024-05-08},
  abstract = {Traffic prediction is significantly important for performance analysis and network planning in Software Defined Networking (SDN). However, to effectively predict network traffic in current networks is very difficult and nearly prohibitive. As a new cutting-edge network technology, SDN decouples the control and data planes of network switch devices to enable the flexibility of network measurements and managements. The SDN architecture of the flow-based forwarding idea brings forth a promising of network traffic capture and prediction. We propose a lightweight traffic prediction algorithm for SDN applications. Firstly, different from traditional network traffic measurements, our method uses the flow-based forwarding idea in SDN to extract traffic statistic from data plane. The statistical variable describes network flow information forwarded in SDN and enables more accurate measurements of flow traffic via a direct and low-overhead way compared with traditional traffic measurements. Secondly, based on the temporal nature of traffic, the time-correlation theory is utilized to model flow traffic, where the time-series analysis theory and regressive modeling approach are used to characterize network traffic in SDN. A fully new method is proposed to perform traffic prediction. Thirdly, we propose the flow-based forwarding traffic prediction algorithm to forecast to SDN traffic. The detailed algorithm process is discussed and analyze. Finally, sufficient experiments are presented and designed to validate the proposed method. Simulation results show that our method is feasible and effective.},
  langid = {english},
  keywords = {Network measurements,Regressive model,Simulation analysis,Software defined networking,Traffic prediction}
}

@article{rusekRouteNetLeveragingGraph2020a,
  title = {{{RouteNet}}: {{Leveraging Graph Neural Networks}} for Network Modeling and Optimization in {{SDN}}},
  shorttitle = {{{RouteNet}}},
  author = {Rusek, Krzysztof and {Su{\'a}rez-Varela}, Jos{\'e} and Almasan, Paul and {Barlet-Ros}, Pere and {Cabellos-Aparicio}, Albert},
  year = {2020},
  month = oct,
  journal = {IEEE Journal on Selected Areas in Communications},
  volume = {38},
  number = {10},
  eprint = {1910.01508},
  primaryclass = {cs},
  pages = {2260--2270},
  issn = {0733-8716, 1558-0008},
  doi = {10.1109/JSAC.2020.3000405},
  urldate = {2024-05-08},
  abstract = {Network modeling is a key enabler to achieve efficient network operation in future self-driving Software-Defined Networks. However, we still lack functional network models able to produce accurate predictions of Key Performance Indicators (KPI) such as delay, jitter or loss at limited cost. In this paper we propose RouteNet, a novel network model based on Graph Neural Network (GNN) that is able to understand the complex relationship between topology, routing, and input traffic to produce accurate estimates of the per-source/destination per-packet delay distribution and loss. RouteNet leverages the ability of GNNs to learn and model graph-structured information and as a result, our model is able to generalize over arbitrary topologies, routing schemes and traffic intensity. In our evaluation, we show that RouteNet is able to predict accurately the delay distribution (mean delay and jitter) and loss even in topologies, routing and traffic unseen in the training (worst case MRE=15.4\%). Also, we present several use cases where we leverage the KPI predictions of our GNN model to achieve efficient routing optimization and network planning.},
  archiveprefix = {arxiv},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Machine Learning,Computer Science - Networking and Internet Architecture},
  file = {C:\Users\lwx1222086\Zotero\storage\QNW9UZJL\Rusek et al. - 2020 - RouteNet Leveraging Graph Neural Networks for net.pdf}
}

@article{pourgheblehComprehensiveSystematicReview2020,
  title = {A Comprehensive and Systematic Review of the Load Balancing Mechanisms in the {{Internet}} of {{Things}}},
  author = {Pourghebleh, Behrouz and Hayyolalam, Vahideh},
  year = {2020},
  month = jun,
  journal = {Cluster Computing},
  volume = {23},
  number = {2},
  pages = {641--661},
  issn = {1573-7543},
  doi = {10.1007/s10586-019-02950-0},
  urldate = {2024-05-08},
  abstract = {The Internet of Things (IoT) is a network of different objects that refers to an environment in which intelligent devices around us can connect to the Internet and exchange information together. A large number of generated events from IoT objects causes overhead on the network. Therefore, to optimize the usage of IoT network, it is essential to provide solutions for network problems including scalability, routing, reliability, security, energy conservation, network lifetime, congestion, heterogeneity, and quality of service (QoS). In this regard, load balancing as an efficient method takes a significant role in distributing loads among different routes. Imbalance traffic load across the network causes high latency in some routes and loss of data packets and decreases packet delivery ratio. Although load balancing has a critical importance in the IoT, there is still a lack of an organized and comprehensive review about analyzing and examining its remarkable methods. Therefore, this paper by adopting a systematic manner aims to address this gap. In this research, the load balancing methods are categorized into two main categories including centralized and distributed and their merits and demerits are specified. Moreover, vital parameters, the challenges, and open issues in this scope are also discussed. Thus, future authors will be able to develop more effective load balancing mechanisms.},
  langid = {english},
  keywords = {Internet of Things,IoT,Load balancing,SLR,Survey,Systematic review}
}

@inproceedings{liuPolicyLearningConstraints2021,
  title = {Policy {{Learning}} with {{Constraints}} in {{Model-free Reinforcement Learning}}: {{A Survey}}},
  shorttitle = {Policy {{Learning}} with {{Constraints}} in {{Model-free Reinforcement Learning}}},
  booktitle = {Proceedings of the {{Thirtieth International Joint Conference}} on {{Artificial Intelligence}}},
  author = {Liu, Yongshuai and Halev, Avishai and Liu, Xin},
  year = {2021},
  month = aug,
  pages = {4508--4515},
  publisher = {International Joint Conferences on Artificial Intelligence Organization},
  address = {Montreal, Canada},
  doi = {10.24963/ijcai.2021/614},
  urldate = {2023-02-01},
  abstract = {Reinforcement Learning (RL) algorithms have had tremendous success in simulated domains. These algorithms, however, often cannot be directly applied to physical systems, especially in cases where there are constraints to satisfy (e.g. to ensure safety or limit resource consumption). In standard RL, the agent is incentivized to explore any policy with the sole goal of maximizing reward; in the real world, however, ensuring satisfaction of certain constraints in the process is also necessary and essential. In this article, we overview existing approaches addressing constraints in model-free reinforcement learning. We model the problem of learning with constraints as a Constrained Markov Decision Process and consider two main types of constraints: cumulative and instantaneous. We summarize existing approaches and discuss their pros and cons. To evaluate policy performance under constraints, we introduce a set of standard benchmarks and metrics. We also summarize limitations of current methods and present open questions for future research.},
  isbn = {978-0-9992411-9-6},
  langid = {english},
  keywords = {read},
  file = {C:\Users\lwx1222086\Zotero\storage\YQTJB77Z\Liu et al. - 2021 - Policy Learning with Constraints in Model-free Rei.pdf}
}

@article{tobagiPerformanceAnalysisCarrier1980,
  title = {Performance Analysis of Carrier Sense Multiple Access with Collision Detection},
  author = {Tobagi, Fouad A and Bruce Hunt, V},
  year = {1980},
  month = oct,
  journal = {Computer Networks (1976)},
  series = {Selected {{Papers}} from the {{First Symposium}} on {{Local}} Area {{Communications Networks}}},
  volume = {4},
  number = {5},
  pages = {245--259},
  issn = {0376-5075},
  doi = {10.1016/0376-5075(80)90014-8},
  urldate = {2024-05-15},
  abstract = {Packet broadcasting in computer communication is attractive in that it combines the advantages of both packet-switching and broadcast communication. All stations share a common channel which is multi-accessed in some random fashion. Among the various random access schemes known, carrier sense multiple access (CSMA) has been shown to be highly efficient for environmen with relatively short propagation delay. Packet broadcasting (and in particular CSMA) has been successfully applied to coaxial cables thus providing an efficient means for communication in local environments. In addition, in such environments the possibility of detecting collisions on the coaxial cable enhances the performance of CSMA by aborting conflicting transmissions, thus giving rise to the carrier sense multiple access schemes with collision detection (CSMA-CD). In this paper we extend an analysis of CSMA to accommodate collision detection. The analysis provides the throughput-delay performance of CSMA-CD and its dependence on such key system parameters as the average retransmission delay and the collision recovery time.}
}

@article{wangCOPETrafficEngineering2006,
  title = {{{COPE}}: Traffic Engineering in Dynamic Networks},
  shorttitle = {{{COPE}}},
  author = {Wang, Hao and Xie, Haiyong and Qiu, Lili and Yang, Yang Richard and Zhang, Yin and Greenberg, Albert},
  year = {2006},
  month = aug,
  journal = {ACM SIGCOMM Computer Communication Review},
  volume = {36},
  number = {4},
  pages = {99--110},
  issn = {0146-4833},
  doi = {10.1145/1151659.1159926},
  urldate = {2024-05-15},
  abstract = {Traffic engineering plays a critical role in determining the performance and reliability of a network. A major challenge in traffic engineering is how to cope with dynamic and unpredictable changes in traffic demand. In this paper, we propose COPE, a class of traffic engineering algorithms that optimize for the expected scenarios while providing a worst-case guarantee for unexpected scenarios. Using extensive evaluations based on real topologies and traffic traces, we show that COPE can achieve efficient resource utilization and avoid network congestion in a wide variety of scenarios.},
  keywords = {COPE,oblivious routing,optimization,traffic engineering,unpredictable traffic},
  file = {C:\Users\lwx1222086\Zotero\storage\HJCCWTEQ\Wang et al. - 2006 - COPE traffic engineering in dynamic networks.pdf}
}

@inproceedings{kumarSemiobliviousTrafficEngineering2018,
  title = {Semi-Oblivious Traffic Engineering: The Road Not Taken},
  shorttitle = {Semi-Oblivious Traffic Engineering},
  booktitle = {Proceedings of the 15th {{USENIX Conference}} on {{Networked Systems Design}} and {{Implementation}}},
  author = {Kumar, Praveen and Yuan, Yang and Yu, Chris and Foster, Nate and Kleinberg, Robert and Lapukhov, Petr and Lim, Chiun Lin and Soul{\'e}, Robert},
  year = {2018},
  month = apr,
  series = {{{NSDI}}'18},
  pages = {157--170},
  publisher = {USENIX Association},
  address = {USA},
  urldate = {2024-05-15},
  abstract = {Networks are expected to provide reliable performance under a wide range of operating conditions, but existing traffic engineering (TE) solutions optimize for performance or robustness, but not both. A key factor that impacts the quality of a TE system is the set of paths used to carry traffic. Some systems rely on shortest paths, which leads to excessive congestion in topologies with bottleneck links, while others use paths that minimize congestion, which are brittle and prone to failure. This paper presents a system that uses a set of paths computed using R{\"a}cke's oblivious routing algorithm, as well as a centralized controller to dynamically adapt sending rates. Although oblivious routing and centralized TE have been studied previously in isolation, their combination is novel and powerful. We built a software framework to model TE solutions and conducted extensive experiments across a large number of topologies and scenarios, including the production backbone of a large content provider and an ISP. Our results show that semi-oblivious routing provides near-optimal performance and is far more robust than state-of-the-art systems.},
  isbn = {978-1-931971-43-0}
}


@inproceedings{anticObliviousRoutingScheme2008,
  title = {Oblivious {{Routing Scheme Using Load Balancing Over Shortest Paths}}},
  booktitle = {2008 {{IEEE International Conference}} on {{Communications}}},
  author = {Antic, M. and Smiljanic, A.},
  year = {2008},
  month = may,
  pages = {5783--5787},
  issn = {1938-1883},
  doi = {10.1109/ICC.2008.1082},
  urldate = {2024-05-15},
  abstract = {In this paper, we propose the oblivious routing scheme based on shortest-path routing and load balancing. We present the LP model that finds the optimal routing. Then we compare the performance of the proposed scheme with the performance of the shortest-path routing for some regular and real-case network topologies. We show that the proposed routing strategy allows to achieve higher guaranteed traffic from/to a node in the network, compared to the case of the classical shortest-path routing.},
  keywords = {Communications Society,Linear programming,Load management,Network topology,Peer to peer computing,Polynomials,Routing,Telecommunication traffic,Throughput,Traffic control}
}

@inproceedings{tsunodaLoadBalancedShortestPathBasedRouting2011,
  title = {Load-{{Balanced Shortest-Path-Based Routing}} without {{Traffic Splitting}} in {{Hose Model}}},
  booktitle = {2011 {{IEEE International Conference}} on {{Communications}} ({{ICC}})},
  author = {Tsunoda, Shunichi and Muktadir, Abu Hena Al and Oki, Eiji},
  year = {2011},
  month = jun,
  pages = {1--5},
  issn = {1938-1883},
  doi = {10.1109/icc.2011.5962963},
  urldate = {2024-05-15},
  abstract = {Smart OSPF (S-OSPF), a load balancing, shortest-path-based routing scheme, was introduced to improve the routing performances of legacy networks running OSPF with known traffic demands. S-OSPF distributes traffic from a source node to neighbor nodes, and, after reaching the neighbor nodes, traffic is routed according to the OSPF protocol. However, in practice, exact traffic demands are difficult to obtain, and most routers will not be able to handle the complexity of determining and implementing uneven traffic distributions with any form of precision. This paper investigates non-split S-OSPF with the hose model for the first time; its goal is to minimize the worst-case network congestion ratio. In this model, traffic from a source node to a destination node is not split over multiple routes, in other words, it goes via only one neighbor node to the destination node. The routing decision problem with the hose model is formulated as an integer linear programming (ILP) problem. Since it is difficult to solve the ILP problem in practical time, this paper proposes a heuristic algorithm. In the routing decision process, the proposed algorithm gives the highest priority to the node pair that has the highest product of ingress and egress traffic, and enables a source node to select the neighbor node that minimizes the maximum link utilization over all links for the worst case traffic condition specified by the hose model. We compare non-split S-OSPF to split S-OSPF and classical shortest path routing (SPR). Numerical results show that the non-split S-OSPF scheme improves routing performance versus classical SPR and is comparable to the split S-OSPF scheme for larger networks.},
  keywords = {Heuristic algorithms,Hoses,IP networks,Load modeling,Peer to peer computing,Routing,Routing protocols},
  file = {C:\Users\lwx1222086\Zotero\storage\8A8ZWXQF\Tsunoda et al_2011_Load-Balanced Shortest-Path-Based Routing without Traffic Splitting in Hose.pdf}
}



@misc{kumarKulfiRobustTraffic2016a,
  title = {Kulfi: {{Robust Traffic Engineering Using Semi-Oblivious Routing}}},
  shorttitle = {Kulfi},
  author = {Kumar, Praveen and Yuan, Yang and Yu, Chris and Foster, Nate and Kleinberg, Robert and Soul{\'e}, Robert},
  year = {2016},
  month = mar,
  number = {arXiv:1603.01203},
  eprint = {1603.01203},
  primaryclass = {cs},
  publisher = {arXiv},
  urldate = {2024-05-15},
  abstract = {Wide-area network traffic engineering enables network operators to reduce congestion and improve utilization by balancing load across multiple paths. Current approaches to traffic engineering can be modeled in terms of a routing component that computes forwarding paths, and a load balancing component that maps incoming flows onto those paths dynamically, adjusting sending rates to fit current conditions. Unfortunately, existing systems rely on simple strategies for one or both of these components, which leads to poor performance or requires making frequent updates to forwarding paths, significantly increasing management complexity. This paper explores a different approach based on semi-oblivious routing, a natural extension of oblivious routing in which the system computes a diverse set of paths independent of demands, but also dynamically adapts sending rates as conditions change. Semi-oblivious routing has a number of important advantages over competing approaches including low overhead, nearly optimal performance, and built-in protection against unexpected bursts of traffic and failures. Through in-depth simulations and a deployment on SDN hardware, we show that these benefits are robust, and hold across a wide range of topologies, demands, resource budgets, and failure scenarios.},
  archiveprefix = {arxiv},
  langid = {english},
  keywords = {C.2.2,C.2.3,C.2.5,C.2.6,C.4,Computer Science - Networking and Internet Architecture},
  file = {C:\Users\lwx1222086\Zotero\storage\KGFXBAL7\Kumar et al. - 2016 - Kulfi Robust Traffic Engineering Using Semi-Obliv.pdf}
}

@article{zhuangComprehensiveSurveyTransfer2020,
  title = {A {{Comprehensive Survey}} on {{Transfer Learning}}},
  author = {Zhuang, Fuzhen and Qi, Zhiyuan and Duan, Keyu and Xi, Dongbo and Zhu, Yongchun and Zhu, Hengshu and Xiong, Hui and He, Qing},
  year = {2020},
  month = jun,
  number = {arXiv:1911.02685},
  eprint = {1911.02685},
  primaryclass = {cs, stat},
  publisher = {arXiv},
  doi = {10.48550/arXiv.1911.02685},
  urldate = {2024-05-16},
  journal      = {CoRR},
  volume       = {abs/1911.02685},
  eprinttype    = {arXiv},
  timestamp    = {Sat, 29 Aug 2020 18:19:14 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/abs-1911-02685.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org},
  abstract = {Transfer learning aims at improving the performance of target learners on target domains by transferring the knowledge contained in different but related source domains. In this way, the dependence on a large number of target domain data can be reduced for constructing target learners. Due to the wide application prospects, transfer learning has become a popular and promising area in machine learning. Although there are already some valuable and impressive surveys on transfer learning, these surveys introduce approaches in a relatively isolated way and lack the recent advances in transfer learning. Due to the rapid expansion of the transfer learning area, it is both necessary and challenging to comprehensively review the relevant studies. This survey attempts to connect and systematize the existing transfer learning researches, as well as to summarize and interpret the mechanisms and the strategies of transfer learning in a comprehensive way, which may help readers have a better understanding of the current research status and ideas. Unlike previous surveys, this survey paper reviews more than forty representative transfer learning approaches, especially homogeneous transfer learning approaches, from the perspectives of data and model. The applications of transfer learning are also briefly introduced. In order to show the performance of different transfer learning models, over twenty representative transfer learning models are used for experiments. The models are performed on three different datasets, i.e., Amazon Reviews, Reuters-21578, and Office-31. And the experimental results demonstrate the importance of selecting appropriate transfer learning models for different applications in practice.},
  archiveprefix = {arxiv},
  keywords = {Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {C:\Users\lwx1222086\Zotero\storage\VVYVIIRL\Zhuang et al. - 2020 - A Comprehensive Survey on Transfer Learning.pdf}
}

@article{liuKANKolmogorovArnoldNetworks2024,
  title = {{{KAN}}: {{Kolmogorov-Arnold Networks}}},
  shorttitle = {{{KAN}}},
  author = {Liu, Ziming and Wang, Yixuan and Vaidya, Sachin and Ruehle, Fabian and Halverson, James and Solja{\v c}i{\'c}, Marin and Hou, Thomas Y. and Tegmark, Max},
  year = {2024},
  month = may,
  journal      = { Computing Research Repository (CoRR)},
  number = {arXiv:2404.19756},
  eprint = {2404.19756},
  primaryclass = {cond-mat, stat},
  publisher = {arXiv},
  doi = {10.48550/arXiv.2404.19756},
  urldate = {2024-05-16},
  abstract = {Inspired by the Kolmogorov-Arnold representation theorem, we propose Kolmogorov-Arnold Networks (KANs) as promising alternatives to Multi-Layer Perceptrons (MLPs). While MLPs have fixed activation functions on nodes ("neurons"), KANs have learnable activation functions on edges ("weights"). KANs have no linear weights at all -- every weight parameter is replaced by a univariate function parametrized as a spline. We show that this seemingly simple change makes KANs outperform MLPs in terms of accuracy and interpretability. For accuracy, much smaller KANs can achieve comparable or better accuracy than much larger MLPs in data fitting and PDE solving. Theoretically and empirically, KANs possess faster neural scaling laws than MLPs. For interpretability, KANs can be intuitively visualized and can easily interact with human users. Through two examples in mathematics and physics, KANs are shown to be useful collaborators helping scientists (re)discover mathematical and physical laws. In summary, KANs are promising alternatives for MLPs, opening opportunities for further improving today's deep learning models which rely heavily on MLPs.},
  archiveprefix = {arxiv},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Machine Learning,Condensed Matter - Disordered Systems and Neural Networks,Statistics - Machine Learning},
  file = {C:\Users\lwx1222086\Zotero\storage\UQEZSKR5\Liu et al_2024_KAN.pdf}
}

@article{wuComprehensiveSurveyGraph2021,
  title = {A {{Comprehensive Survey}} on {{Graph Neural Networks}}},
  author = {Wu, Zonghan and Pan, Shirui and Chen, Fengwen and Long, Guodong and Zhang, Chengqi and Yu, Philip S.},
  year = {2021},
  month = jan,
  journal = {IEEE Transactions on Neural Networks and Learning Systems},
  volume = {32},
  number = {1},
  eprint = {1901.00596},
  primaryclass = {cs, stat},
  pages = {4--24},
  issn = {2162-237X, 2162-2388},
  doi = {10.1109/TNNLS.2020.2978386},
  urldate = {2024-05-16},
  abstract = {Deep learning has revolutionized many machine learning tasks in recent years, ranging from image classification and video processing to speech recognition and natural language understanding. The data in these tasks are typically represented in the Euclidean space. However, there is an increasing number of applications where data are generated from non-Euclidean domains and are represented as graphs with complex relationships and interdependency between objects. The complexity of graph data has imposed significant challenges on existing machine learning algorithms. Recently, many studies on extending deep learning approaches for graph data have emerged. In this survey, we provide a comprehensive overview of graph neural networks (GNNs) in data mining and machine learning fields. We propose a new taxonomy to divide the state-of-the-art graph neural networks into four categories, namely recurrent graph neural networks, convolutional graph neural networks, graph autoencoders, and spatial-temporal graph neural networks. We further discuss the applications of graph neural networks across various domains and summarize the open source codes, benchmark data sets, and model evaluation of graph neural networks. Finally, we propose potential research directions in this rapidly growing field.},
  archiveprefix = {arxiv},
  keywords = {Computer Science - Machine Learning,Statistics - Machine Learning}
}

@inproceedings{valadarskyLearningRoute2017,
  title = {Learning to {{Route}}},
  booktitle = {Proceedings of the 16th {{ACM Workshop}} on {{Hot Topics}} in {{Networks}}},
  author = {Valadarsky, Asaf and Schapira, Michael and Shahaf, Dafna and Tamar, Aviv},
  year = {2017},
  month = nov,
  pages = {185--191},
  publisher = {ACM},
  address = {Palo Alto CA USA},
  doi = {10.1145/3152434.3152441},
  urldate = {2024-05-17},
  abstract = {Recently, much attention has been devoted to the question of whether/when traditional network protocol design, which relies on the application of algorithmic insights by human experts, can be replaced by a data-driven (i.e., machine learning) approach. We explore this question in the context of the arguably most fundamental networking task: routing. Can ideas and techniques from machine learning (ML) be leveraged to automatically generate ``good'' routing configurations? We focus on the classical setting of intradomain traffic engineering. We observe that this context poses significant challenges for data-driven protocol design. Our preliminary results regarding the power of data-driven routing suggest that applying ML (specifically, deep reinforcement learning) to this context yields high performance and is a promising direction for further research. We outline a research agenda for ML-guided routing.},
  isbn = {978-1-4503-5569-8},
  langid = {english},
  file = {C:\Users\lwx1222086\Zotero\storage\MVTWLCPI\Valadarsky et al. - 2017 - Learning to Route.pdf}
}

@inproceedings{rackeMinimizingCongestionGeneral2002a,
  title = {Minimizing Congestion in General Networks},
  booktitle = {The 43rd {{Annual IEEE Symposium}} on {{Foundations}} of {{Computer Science}}, 2002. {{Proceedings}}.},
  author = {Racke, H.},
  year = {2002},
  month = nov,
  pages = {43--52},
  issn = {0272-5428},
  doi = {10.1109/SFCS.2002.1181881},
  urldate = {2024-05-17},
  abstract = {A principle task in parallel and distributed systems is to reduce the communication load in the interconnection network, as this is usually the major bottleneck for the performance of distributed applications. We introduce a framework for solving online problems that aim to minimize the congestion (i.e. the maximum load of a network link) in general topology networks. We apply this framework to the problem of online routing of virtual circuits and to a dynamic data management problem. For both scenarios we achieve a competitive ratio of O(log/sup 3/ n) with respect to the congestion of the network links. Our online algorithm for the routing problem has the remarkable property that it is oblivious, i.e., the path chosen for a virtual circuit is independent of the current network load. Oblivious routing strategies can easily be implemented in distributed environments and have therefore been intensively studied for certain network topologies as e.g. meshes, tori and hypercubic networks. This is the first oblivious path selection algorithm that achieves a polylogarithmic competitive ratio in general networks.},
  keywords = {Application software,Bandwidth,Circuit topology,Computer science,Intelligent networks,Mathematics,Multiprocessor interconnection networks,Network topology,Routing,Workstations}
}

@inproceedings{perryDOTERethinkingPredictive2023a,
  title = {{DOTE: Rethinking Predictive WAN Traffic Engineering}},
  shorttitle = {\{\vphantom\}{{DOTE}}\vphantom\{\}},
  booktitle = {20th {{USENIX Symposium}} on {{Networked Systems Design}} and {{Implementation}} ({{NSDI}} 23)},
  author = {Perry, Yarin and Frujeri, Felipe Vieira and Hoch, Chaim and Kandula, Srikanth and Menache, Ishai and Schapira, Michael and Tamar, Aviv},
  year = {2023},
  pages = {1557--1581},
  urldate = {2024-05-17},
  isbn = {978-1-939133-33-5},
  langid = {english},
  file = {C:\Users\lwx1222086\Zotero\storage\896TVHWE\Perry et al. - 2023 - DOTE Rethinking (Predictive) WAN Traffic Engi.pdf}
}

@article{wachiSafeReinforcementLearning2020a,
  title = {Safe {{Reinforcement Learning}} in {{Constrained Markov Decision Processes}}},
  author = {Wachi, Akifumi and Sui, Yanan},
  year = {2020},
  month = aug,
  number = {arXiv:2008.06626},
  eprint = {2008.06626},
  primaryclass = {cs},
  publisher = {arXiv},
  doi = {10.48550/arXiv.2008.06626},
  urldate = {2023-02-01},
  journal      = { Computing Research Repository (CoRR)},
  abstract = {Safe reinforcement learning has been a promising approach for optimizing the policy of an agent that operates in safety-critical applications. In this paper, we propose an algorithm, SNO-MDP, that explores and optimizes Markov decision processes under unknown safety constraints. Specifically, we take a stepwise approach for optimizing safety and cumulative reward. In our method, the agent first learns safety constraints by expanding the safe region, and then optimizes the cumulative reward in the certified safe region. We provide theoretical guarantees on both the satisfaction of the safety constraint and the near-optimality of the cumulative reward under proper regularity assumptions. In our experiments, we demonstrate the effectiveness of SNO-MDP through two experiments: one uses a synthetic data in a new, openly-available environment named GP-SAFETY-GYM, and the other simulates Mars surface exploration by using real observation data.},
  archiveprefix = {arxiv},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Machine Learning,Computer Science - Robotics,read},
  file = {C:\Users\lwx1222086\Zotero\storage\FEJIAC9D\Wachi_Sui_2020_Safe Reinforcement Learning in Constrained Markov Decision Processes.pdf}
}

@article{zhangSurveyNeuralNetwork2021,
  title = {A {{Survey}} on {{Neural Network Interpretability}}},
  author = {Zhang, Yu and Ti{\v n}o, Peter and Leonardis, Ale{\v s} and Tang, Ke},
  year = {2021},
  month = oct,
  journal = {IEEE Transactions on Emerging Topics in Computational Intelligence},
  volume = {5},
  number = {5},
  pages = {726--742},
  issn = {2471-285X},
  doi = {10.1109/TETCI.2021.3100641},
  urldate = {2024-05-17},
  abstract = {Along with the great success of deep neural networks, there is also growing concern about their black-box nature. The interpretability issue affects people's trust on deep learning systems. It is also related to many ethical problems, e.g., algorithmic discrimination. Moreover, interpretability is a desired property for deep networks to become powerful tools in other research fields, e.g., drug discovery and genomics. In this survey, we conduct a comprehensive review of the neural network interpretability research. We first clarify the definition of interpretability as it has been used in many different contexts. Then we elaborate on the importance of interpretability and propose a novel taxonomy organized along three dimensions: type of engagement (passive vs. active interpretation approaches), the type of explanation, and the focus (from local to global interpretability). This taxonomy provides a meaningful 3D view of distribution of papers from the relevant literature as two of the dimensions are not simply categorical but allow ordinal subcategories. Finally, we summarize the existing interpretability evaluation methods and suggest possible research directions inspired by our new taxonomy.},
  keywords = {Decision trees,Deep learning,inter-pretability,Machine learning,neural networks,Reliability,survey,Task analysis,Taxonomy,Tools,Training}
}

@inproceedings{wangSurveyInterpretableMachine2022,
  title = {A {{Survey}} of {{Interpretable Machine Learning Methods}}},
  booktitle = {2022 {{International Conference}} on {{Virtual Reality}}, {{Human-Computer Interaction}} and {{Artificial Intelligence}} ({{VRHCIAI}})},
  author = {Wang, Yan and Tuerhong, Gulanbaier},
  year = {2022},
  month = oct,
  pages = {232--237},
  doi = {10.1109/VRHCIAI57205.2022.00047},
  abstract = {Recently, people are increasingly pursuing more accurate machine learning systems. At the same time, the problem is that it is difficult for people to understand the internal logical structure of the system, and the machine learning model has become a black box. Lack of explanation is not only a practical problem, but also an ethical problem. At this point, understanding why a model makes a prediction is as important as the accuracy of the prediction. In order to balance the interpretability and accuracy of the model, many experts and scholars have done a lot of research on improving the interpretability of machine learning model, improved the interpretability of the model from different dimensions, and created a series of interpretable methods to help users understand the internal logic of the system and make the black box transparent. However, the current interpretability research is still in the stage of development, and there is no completely unified interpretable method at present. In this paper, firstly, the development status of machine learning and the importance of interpretable learning are discussed. Then, according to the current research status, interpretable methods are introduced from interpretable models and model independent categories, the research and application in the field of interpretability are discussed, and the current challenges and future development of interpretability are analyzed, To further promote the research and development of interpretability.},
  keywords = {Analytical models,black box component,Ethics,Human computer interaction,interpretability,interpretable methods,machine learning,Machine learning,Predictive models,Solid modeling,Virtual reality},
  file = {C\:\\Users\\lwx1222086\\Zotero\\storage\\XZSX4CHK\\Wang_Tuerhong_2022_A Survey of Interpretable Machine Learning Methods.pdf;C\:\\Users\\lwx1222086\\Zotero\\storage\\86J6QJBS\\10062911.html}
}



@inproceedings{ribeiroWhyShouldTrust2016,
  title = {"{{Why Should I Trust You}}?": {{Explaining}} the {{Predictions}} of {{Any Classifier}}},
  shorttitle = {"{{Why Should I Trust You}}?},
  booktitle = {Proceedings of the 22nd {{ACM SIGKDD International Conference}} on {{Knowledge Discovery}} and {{Data Mining}}},
  author = {Ribeiro, Marco Tulio and Singh, Sameer and Guestrin, Carlos},
  year = {2016},
  month = aug,
  series = {{{KDD}} '16},
  pages = {1135--1144},
  publisher = {Association for Computing Machinery},
  address = {New York, NY, USA},
  doi = {10.1145/2939672.2939778},
  urldate = {2024-05-17},
  abstract = {Despite widespread adoption, machine learning models remain mostly black boxes. Understanding the reasons behind predictions is, however, quite important in assessing trust, which is fundamental if one plans to take action based on a prediction, or when choosing whether to deploy a new model. Such understanding also provides insights into the model, which can be used to transform an untrustworthy model or prediction into a trustworthy one. In this work, we propose LIME, a novel explanation technique that explains the predictions of any classifier in an interpretable and faithful manner, by learning an interpretable model locally varound the prediction. We also propose a method to explain models by presenting representative individual predictions and their explanations in a non-redundant way, framing the task as a submodular optimization problem. We demonstrate the flexibility of these methods by explaining different models for text (e.g. random forests) and image classification (e.g. neural networks). We show the utility of explanations via novel experiments, both simulated and with human subjects, on various scenarios that require trust: deciding if one should trust a prediction, choosing between models, improving an untrustworthy classifier, and identifying why a classifier should not be trusted.},
  isbn = {978-1-4503-4232-2},
  keywords = {black box classifier,explaining machine learning,interpretability,interpretable machine learning}
}


@misc{lundbergUnifiedApproachInterpreting2017,
  title = {A {{Unified Approach}} to {{Interpreting Model Predictions}}},
  author = {Lundberg, Scott and Lee, Su-In},
  year = {2017},
  month = nov,
  number = {arXiv:1705.07874},
  eprint = {1705.07874},
  primaryclass = {cs, stat},
  publisher = {arXiv},
journal      = { Computing Research Repository (CoRR)},
  doi = {10.48550/arXiv.1705.07874},
  urldate = {2024-05-17},
  abstract = {Understanding why a model makes a certain prediction can be as crucial as the prediction's accuracy in many applications. However, the highest accuracy for large modern datasets is often achieved by complex models that even experts struggle to interpret, such as ensemble or deep learning models, creating a tension between accuracy and interpretability. In response, various methods have recently been proposed to help users interpret the predictions of complex models, but it is often unclear how these methods are related and when one method is preferable over another. To address this problem, we present a unified framework for interpreting predictions, SHAP (SHapley Additive exPlanations). SHAP assigns each feature an importance value for a particular prediction. Its novel components include: (1) the identification of a new class of additive feature importance measures, and (2) theoretical results showing there is a unique solution in this class with a set of desirable properties. The new class unifies six existing methods, notable because several recent methods in the class lack the proposed desirable properties. Based on insights from this unification, we present new methods that show improved computational performance and/or better consistency with human intuition than previous approaches.},
  archiveprefix = {arxiv},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Machine Learning,Statistics - Machine Learning}
}

@article{scarselliGraphNeuralNetwork2009,
  title = {The {{Graph Neural Network Model}}},
  author = {Scarselli, Franco and Gori, Marco and Tsoi, Ah Chung and Hagenbuchner, Markus and Monfardini, Gabriele},
  year = {2009},
  month = jan,
  journal = {IEEE Transactions on Neural Networks},
  volume = {20},
  number = {1},
  pages = {61--80},
  issn = {1941-0093},
  doi = {10.1109/TNN.2008.2005605},
  urldate = {2024-05-17},
  abstract = {Many underlying relationships among data in several areas of science and engineering, e.g., computer vision, molecular chemistry, molecular biology, pattern recognition, and data mining, can be represented in terms of graphs. In this paper, we propose a new neural network model, called graph neural network (GNN) model, that extends existing neural network methods for processing the data represented in graph domains. This GNN model, which can directly process most of the practically useful types of graphs, e.g., acyclic, cyclic, directed, and undirected, implements a function tau(G,n) isin IRm that maps a graph G and one of its nodes n into an m-dimensional Euclidean space. A supervised learning algorithm is derived to estimate the parameters of the proposed GNN model. The computational cost of the proposed algorithm is also considered. Some experimental results are shown to validate the proposed learning algorithm, and to demonstrate its generalization capabilities.},
  keywords = {Biological system modeling,Biology,Chemistry,Computer vision,Data engineering,Data mining,graph neural networks (GNNs),graph processing,Graphical domains,Neural networks,Parameter estimation,Pattern recognition,recursive neural networks,Supervised learning},
  file = {C:\Users\lwx1222086\Zotero\storage\9P5K3WRM\Scarselli et al. - 2009 - The Graph Neural Network Model.pdf}
}

@article{parkStableFDGStyleAttention2023,
  title = {{{StableFDG}}: {{Style}} and {{Attention Based Learning}} for {{Federated Domain Generalization}}},
  shorttitle = {{{StableFDG}}},
  author = {Park, Jungwuk and Han, Dong-Jun and Kim, Jinho and Wang, Shiqiang and Brinton, Christopher G. and Moon, Jaekyun},
  year = {2023},
  month = oct,
  number = {arXiv:2311.00227},
journal      = { Computing Research Repository (CoRR)},
  eprint = {2311.00227},
  primaryclass = {cs},
  publisher = {arXiv},
  doi = {10.48550/arXiv.2311.00227},
  urldate = {2024-05-17},
  abstract = {Traditional federated learning (FL) algorithms operate under the assumption that the data distributions at training (source domains) and testing (target domain) are the same. The fact that domain shifts often occur in practice necessitates equipping FL methods with a domain generalization (DG) capability. However, existing DG algorithms face fundamental challenges in FL setups due to the lack of samples/domains in each client's local dataset. In this paper, we propose StableFDG, a style and attention based learning strategy for accomplishing federated domain generalization, introducing two key contributions. The first is style-based learning, which enables each client to explore novel styles beyond the original source domains in its local dataset, improving domain diversity based on the proposed style sharing, shifting, and exploration strategies. Our second contribution is an attention-based feature highlighter, which captures the similarities between the features of data samples in the same class, and emphasizes the important/common characteristics to better learn the domain-invariant characteristics of each class in data-poor FL scenarios. Experimental results show that StableFDG outperforms existing baselines on various DG benchmark datasets, demonstrating its efficacy.},
  archiveprefix = {arxiv},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Machine Learning},
  file = {C:\Users\lwx1222086\Zotero\storage\YSWF3Z8L\Park et al. - 2023 - StableFDG Style and Attention Based Learning for .pdf}
}


@article{omidshafieiDeepDecentralizedMultitask2017,
  title = {Deep {{Decentralized Multi-task Multi-Agent Reinforcement Learning}} under {{Partial Observability}}},
  author = {Omidshafiei, Shayegan and Pazis, Jason and Amato, Christopher and How, Jonathan P. and Vian, John},
  year = {2017},
  month = jul,
journal      = { Computing Research Repository (CoRR)},
  number = {arXiv:1703.06182},
  eprint = {1703.06182},
  primaryclass = {cs},
  publisher = {arXiv},
  doi = {10.48550/arXiv.1703.06182},
  urldate = {2024-05-17},
  abstract = {Many real-world tasks involve multiple agents with partial observability and limited communication. Learning is challenging in these settings due to local viewpoints of agents, which perceive the world as non-stationary due to concurrently-exploring teammates. Approaches that learn specialized policies for individual tasks face problems when applied to the real world: not only do agents have to learn and store distinct policies for each task, but in practice identities of tasks are often non-observable, making these approaches inapplicable. This paper formalizes and addresses the problem of multi-task multi-agent reinforcement learning under partial observability. We introduce a decentralized single-task learning approach that is robust to concurrent interactions of teammates, and present an approach for distilling single-task policies into a unified policy that performs well across multiple related tasks, without explicit provision of task identity.},
  archiveprefix = {arxiv},
  keywords = {Computer Science - Artificial Intelligence,Computer Science - Machine Learning,Computer Science - Multiagent Systems}
}

@article{kirkSurveyZeroshotGeneralisation2023a,
  title = {A {{Survey}} of {{Zero-shot Generalisation}} in {{Deep Reinforcement Learning}}},
  author = {Kirk, Robert and Zhang, Amy and Grefenstette, Edward and Rockt{\"a}schel, Tim},
  year = {2023},
  month = may,
  journal = {Journal of Artificial Intelligence Research},
  volume = {76},
  issn = {1076-9757},
  doi = {10.1613/jair.1.14174},
  urldate = {2024-05-19},
  abstract = {The study of zero-shot generalisation (ZSG) in deep Reinforcement Learning (RL) aims to produce RL algorithms whose policies generalise well to novel unseen situations at deployment time, avoiding overfitting to their training environments. Tackling this is vital if we are to deploy reinforcement learning algorithms in real world scenarios, where the environment will be diverse, dynamic and unpredictable. This survey is an overview of this nascent field. We rely on a unifying formalism and terminology for discussing different ZSG problems, building upon previous works. We go on to categorise existing benchmarks for ZSG, as well as current methods for tackling these problems. Finally, we provide a critical discussion of the current state of the field, including recommendations for future work. Among other conclusions, we argue that taking a purely procedural content generation approach to benchmark design is not conducive to progress in ZSG, we suggest fast online adaptation and tackling RL-specific problems as some areas for future work on methods for ZSG, and we recommend building benchmarks in underexplored problem settings such as offline RL ZSG and reward-function variation.}
}

@article{jainB4ExperienceGloballydeployed2013,
  title = {B4: Experience with a Globally-Deployed Software Defined Wan},
  shorttitle = {B4},
  author = {Jain, Sushant and Kumar, Alok and Mandal, Subhasree and Ong, Joon and Poutievski, Leon and Singh, Arjun and Venkata, Subbaiah and Wanderer, Jim and Zhou, Junlan and Zhu, Min and Zolla, Jon and H{\"o}lzle, Urs and Stuart, Stephen and Vahdat, Amin},
  year = {2013},
  month = aug,
  journal = {ACM SIGCOMM Computer Communication Review},
  volume = {43},
  number = {4},
  pages = {3--14},
  issn = {0146-4833},
  doi = {10.1145/2534169.2486019},
  urldate = {2024-05-22},
  abstract = {We present the design, implementation, and evaluation of B4, a private WAN connecting Google's data centers across the planet. B4 has a number of unique characteristics: i) massive bandwidth requirements deployed to a modest number of sites, ii) elastic traffic demand that seeks to maximize average bandwidth, and iii) full control over the edge servers and network, which enables rate limiting and demand measurement at the edge. These characteristics led to a Software Defined Networking architecture using OpenFlow to control relatively simple switches built from merchant silicon. B4's centralized traffic engineering service drives links to near 100\% utilization, while splitting application flows among multiple paths to balance capacity against application priority/demands. We describe experience with three years of B4 production deployment, lessons learned, and areas for future work.},
  keywords = {centralized traffic engineering,openflow,routing,software- defined networking,wide-area networks},
  file = {C:\Users\lwx1222086\Zotero\storage\PPH4VV2D\Jain et al_2013_B4.pdf}
}

@inproceedings{liuTrafficEngineeringForward2014,
  title = {Traffic Engineering with Forward Fault Correction},
  booktitle = {Proceedings of the 2014 {{ACM}} Conference on {{SIGCOMM}}},
  author = {Liu, Hongqiang Harry and Kandula, Srikanth and Mahajan, Ratul and Zhang, Ming and Gelernter, David},
  year = {2014},
  month = aug,
  series = {{{SIGCOMM}} '14},
  pages = {527--538},
  publisher = {Association for Computing Machinery},
  address = {New York, NY, USA},
  doi = {10.1145/2619239.2626314},
  urldate = {2024-05-22},
  abstract = {Faults such as link failures and high switch configuration delays can cause heavy congestion and packet loss. Because it takes time to detect and react to faults, these conditions can last long---even tens of seconds. We propose forward fault correction (FFC), a proactive approach to handling faults. FFC spreads network traffic such that freedom from congestion is guaranteed under arbitrary combinations of up to k faults. We show how FFC can be practically realized by compactly encoding the constraints that arise from this large number of possible faults and solving them efficiently using sorting networks. Experiments with data from real networks show that, with negligible loss in overall network throughput, FFC can reduce data loss by a factor of 7--130 in well-provisioned networks, and reduce the loss of high-priority traffic to almost zero in well-utilized networks.},
  isbn = {978-1-4503-2836-4},
  keywords = {congestion-free,fault tolerance,traffic engineering},
  file = {C:\Users\lwx1222086\Zotero\storage\BI89TUFC\Liu et al_2014_Traffic engineering with forward fault correction.pdf}
}

@inproceedings{rackeMinimizingCongestionGeneral2002b,
  title = {Minimizing {{Congestion}} in {{General Networks}}},
  booktitle = {Proceedings of the 43rd {{Symposium}} on {{Foundations}} of {{Computer Science}}},
  author = {R{\"a}cke, Harald},
  year = {2002},
  month = nov,
  series = {{{FOCS}} '02},
  pages = {43--52},
  publisher = {IEEE Computer Society},
  address = {USA},
  urldate = {2024-05-22},
doi = {10.1109/SFCS.2002.1181881},
  abstract = {A principle task in parallel and distributed systems is to reduce the communication load in the interconnection network, as this is usually the major bottleneck for the performance of distributed applications. In this paper we introduce a framework for solving on-line problems that aim to minimize the congestion (i.e. the maximum load of a network link) in general topology networks.We apply this framework to the problem of on-line routing of virtual circuits and to a dynamic data management problem. For both scenarios we achieve a competitive ratioof O(log3n) with respect to the congestion of the network links.Our on-line algorithm for the routing problem has the remarkable property that it is oblivious, i.e., the path chosen for a virtual circuit is independent of the current network load. Oblivious routing strategies can easily be implemented in distributed environments and have thereforebeen intensively studied for certain network topologies as e.g. meshes, tori and hypercubic networks. This is the first oblivious path selection algorithm that achieves a polylogarithmiccompetitive ratio in general networks.},
  isbn = {978-0-7695-1822-0}
}

@article{dalalsafeexploration2018,
  author       = {Gal Dalal and
                  Krishnamurthy Dvijotham and
                  Matej Vecer{\'{\i}}k and
                  Todd Hester and
                  Cosmin Paduraru and
                  Yuval Tassa},
  title        = {Safe Exploration in Continuous Action Spaces},
  journal      = {Computing Research Repository (CoRR)},
  volume       = {abs/1801.08757},
  year         = {2018},
  eprinttype    = {arXiv},
  eprint       = {1801.08757},
  timestamp    = {Wed, 24 Jul 2019 16:34:28 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/abs-1801-08757.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{haons3ai2020,
author = {Yin, Hao and Liu, Pengyu and Liu, Keshu and Cao, Liu and Zhang, Lytianyang and Gao, Yayu and Hei, Xiaojun},
title = {Ns3-Ai: Fostering Artificial Intelligence Algorithms for Networking Research},
year = {2020},
isbn = {9781450375375},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
doi = {10.1145/3389400.3389404},
booktitle = {Proceedings of the 2020 Workshop on Ns-3},
pages = {57–64},
numpages = {8},
keywords = {AI, network simulation, ns-3},
location = {Gaithersburg, MD, USA},
series = {WNS3 2020}
}

@online{ciscoOverviewNetflow,
  title = {Overview of {{Netflow}}},
  author = {Cisco},
  journal = {Overview of Netflow},
  urldate = {2024-08-12},
  year         = {2024},

  url  = {https://www.cisco.com/products/ios-nx-os-software/ios-netflow/index.html},
  file = {C:\Users\TFPC5753\Zotero\storage\3F8MB77N\fnf-xe-3e-asr920-book.html}
}

@online{huaweiOverviewNetstream,
  title = {Overview of {{Netstream}}},
  author = {Huawei},
  journal = {Overview of Netstream},
  urldate = {2024-08-12},
  year         = {2024},

  url  = {https://info.support.huawei.com/info-finder/encyclopedia/en/NetStream.html},
  file = {C:\Users\TFPC5753\Zotero\storage\3F8MB77N\fnf-xe-3e-asr920-book.html}
}
@online{huaweiIFIT,
  title = {Overview of {{IFIT}}},
  author = {Huawei},
  journal = {Overview of IFIT},
  urldate = {2024-08-12},
  year         = {2024},

  url  = {https://info.support.huawei.com/info-finder/encyclopedia/en/IFIT.html},
}
@online{huaweiNCEIP,
  title = {{iMaster NCE-IP V100R024C00 Product Description}},
  author = {Huawei},
  urldate = {2024-08-12},
  year         = {2024},

  url  = {https://support.huawei.com/enterprise/en/doc/EDOC1100385811},
}

@online{huaweisnmp,
  title = {Overview of {{Simple Network Management Protocol }}},
  author = {Huawei},
  journal = {Overview of Simple Network Management Protocol},
  urldate = {2024-08-12},
  year         = {2024},

  url  = {https://info.support.huawei.com/info-finder/encyclopedia/en/SNMP.html},
  file = {C:\Users\TFPC5753\Zotero\storage\3F8MB77N\fnf-xe-3e-asr920-book.html}
}

@online{ns3web,
  title = {{{NS3 Network Simulator}}},
  author = {Nsnam},
  journal = {{{NS3 Network Simulator}}},
  urldate = {2024-08-12},
  year         = {2024},

  url  = {https://www.nsnam.org/},
  file = {C:\Users\TFPC5753\Zotero\storage\3F8MB77N\fnf-xe-3e-asr920-book.html}
}

@inproceedings{dinhLoadBalancingSafe2024,
  title = {Load {{Balancing}} with {{Safe Reinforcement Learning}}},
  booktitle = {{{CoRes}} 2024: 9{\`e}mes {{Rencontres Francophones}} Sur La {{Conception}} de {{Protocoles}}, l'{{{\'E}valuation}} de {{Performance}} et l'{{Exp{\'e}rimentation}} Des {{R{\'e}seaux}} de {{Communication}}},
  author = {Dinh, Lam and Quang, Pham Tran Anh and Leguay, J{\'e}r{\'e}mie},
  year = {2024},
  month = may,
  address = {Saint-Briac-sur-Mer, France},
  urldate = {2024-09-03},
  abstract = {Deep Reinforcement Learning (DRL) algorithms have recently made significant strides in improving network performance. Nonetheless, their practical use is still limited in the absence of safe exploration and safe decision-making. In the context of commercial solutions, reliable and safe-to-operate systems are of paramount importance. Taking this problem into account, we propose a safe learning-based load balancing algorithm for Software Defined-Wide Area Network (SD-WAN), which is empowered by Deep Reinforcement Learning (DRL) combined with a Control Barrier Function (CBF). It safely projects unsafe actions into feasible ones during both training and testing, and it guides learning towards safe policies. We successfully implemented the solution on GPU to accelerate training by approximately 110x times and achieve model updates for on-policy methods within a few seconds, making the solution practical. We show that our approach delivers near-optimal Quality-of-Service (QoS performance in terms of end-to-end delay while respecting safety requirements related to link capacity constraints.},
  keywords = {Control Barrier Function (CBF),Deep Reinforcement Learning (DRL),Software Defined-Wide Area Network (SD-WAN)}
}

@inproceedings{dinhSafeLoadBalancing2024a,
  title = {Towards {{Safe Load Balancing}} Based on {{Control Barrier Functions}} and {{Deep Reinforcement Learning}}},
  booktitle = {{{NOMS}} 2024-2024 {{IEEE Network Operations}} and {{Management Symposium}}},
  author = {Dinh, Lam and Quang, Pham Tran Anh and Leguay, J{\'e}r{\'e}mie},
  year = {2024},
  month = may,
  pages = {1--9},
  issn = {2374-9709},
  doi = {10.1109/NOMS59830.2024.10575399},
  urldate = {2024-09-03},
  abstract = {Deep Reinforcement Learning (DRL) algorithms have recently made significant strides in improving network performance. Nonetheless, their practical use is still limited in the absence of safe exploration and safe decision-making. In the context of commercial solutions, reliable and safe-to-operate systems are of paramount importance. Taking this problem into account, we propose a safe learning-based load balancing algorithm for Software Defined-Wide Area Network (SD-WAN), which is empowered by Deep Reinforcement Learning (DRL) combined with a Control Barrier Function (CBF). It safely projects unsafe actions into feasible ones during both training and testing, and it guides learning towards safe policies. We successfully implemented the solution on GPU to accelerate training by approximately 110x times and achieve model updates for on-policy methods within a few seconds, making the solution practical. We show that our approach delivers near-optimal Quality-of-Service (QoS) performance in terms of end-to-end delay while respecting safety requirements related to link capacity constraints. We also demonstrated that on-policy learning based on Proximal Policy Optimization (PPO) performs better than off-policy learning with Deep Deterministic Policy Gradient (DDPG) when both are combined with a CBF for safe load balancing.},
  keywords = {Control Barrier Function (CBF),Deep reinforcement learning,Deep Reinforcement Learning (DRL),Graphics processing units,Load management,Quality of service,Safety,Software,Software Defined-Wide Area Network (SD-WAN),Training},
  file = {C:\Users\TFPC5753\Zotero\storage\9MF7T5ZN\10575399.html}
}

